Diagonalisation SGD: Fast & Convergent SGD for Non-Differentiable Models via Reparameterisation and Smoothing

It is well-known that the reparameterisation gradient estimator, which exhibits low variance in practice, is biased for non-differentiable models. This may compromise correctness of gradient-based optimisation methods such as stochastic gradient descent (SGD). We introduce a simple syntactic framework to define non-differentiable functions piecewisely and present a systematic approach to obtain smoothings for which the reparameterisation gradient estimator is unbiased. Our main contribution is a novel variant of SGD, Diagonalisation Stochastic Gradient Descent, which progressively enhances the accuracy of the smoothed approximation during optimisation, and we prove convergence to stationary points of the unsmoothed (original) objective. Our empirical evaluation reveals benefits over the state of the art: our approach is simple, fast, stable and attains orders of magnitude reduction in work-normalised variance.

==> apx-experiments.tex <==
% !TEX root = ./main.tex

\paragraph{Results for publicly available code from \cite{LYY18}}

Building on the Python implementation of black-box variational inference given
in \citet{LYY18}, we implement our smoothed gradient estimator and re-run their
experiments with this additional estimator.

The ELBO trajectories are shown in Figure~\ref{fig:lyy-trajectories} and the
work-normalised variance ratios are given in \cref{tab:lyy18-var} in the same
way as in Section~\ref{sec:eval}.

Some discrepancies between our implementation and this likely arise from how the
models are implemented, ours written directly in Python and efficiently
vectorised whereas the ones from \citet{LYY18} are dynamically constructed by parsing
a variant of lambda calculus with little to no optimisation.

The smoothed estimator is also not implemented quite as efficiently here since
there is more overhead for constructing a gradient that explores all of the
branches in their implementation.

Despite this, our smoothed estimator still performs comparably on the ELBO
trajectories and has a smaller work-normalised variance in most situations.

\begin{figure}
  \centering
  \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\columnwidth]{figures/temperature-lyy18.eps}
    \caption{\texttt{temperature}}
  \end{subfigure}
  \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\columnwidth]{figures/textmsg-lyy18.eps}
    \caption{\texttt{textmsg}}
  \end{subfigure}
  \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\columnwidth]{figures/influenza-lyy18.eps}
    \caption{\texttt{influenza}}
  \end{subfigure}
  \caption{ELBO trajectories for each model using the code from \citet{LYY18} for $N=1$.  }
  \label{fig:lyy-trajectories}
\end{figure}

\begin{table}[h]
  \caption{Computational cost and work-normalised variances using the results from the \citet{LYY18} code, all given as ratios with respect to the \textsc{Score} estimator (omitted since it would be all $1$s).}
  \centering
  \label{tab:lyy18-var}

  \vspace*{5pt}
  \begin{subtable}{0.45\linewidth}
    \caption{Temperature}
    \centering
    \begin{small}
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Reparam}  & 1.12e+00   & 5.29e-09   & 2.81e-08\\
      \textsc{Lyy18}    & 1.23e+00   & 1.45e-08   & 5.12e-07\\
      \textsc{Smooth}   & 1.08e+00   & 1.48e-09   & 1.03e-08\\
      \bottomrule
    \end{tabular}
  \end{small}
  \end{subtable}%
  \begin{subtable}{0.45\linewidth}
    \caption{Textmsg}
    \centering
    \begin{small}
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Reparam}  & 1.15e+00   & 2.41e-02   & 2.44e-02\\
      \textsc{Lyy18}    & 1.19e+00   & 3.16e-02   & 2.97e-02\\
      \textsc{Smooth}   & 1.11e+00   & 2.19e-02   & 2.16e-02\\
      \bottomrule
    \end{tabular}
  \end{small}
  \end{subtable}

  \vspace*{10pt}
  \begin{subtable}{0.5\linewidth}
    \caption{Influenza}
    \centering
    \begin{small}
    \begin{tabular}{lcccr}
      \toprule
      Estimator & Cost & $\textrm{Avg}(V(.))$ & $V(\|.\|_2)$ \\
      \midrule
      \textsc{Reparam}  & 2.27e+00   & 1.03e-02   & 4.91e-03  \\
      \textsc{Lyy18}    & 2.41e+00   & 1.23e-02   & 5.83e-03  \\
      \textsc{Smooth}   & 3.63e+00   & 1.61e-02   & 7.77e-03  \\
      \bottomrule
    \end{tabular}
  \end{small}
  \end{subtable}
\end{table}


==> backup.tex <==
\section{Programming Language}
\label{sec:pl}

\changed[dw]{Our starting point is a simple first-order programming language with reals, conditionals, and a non-standard \emph{reparameterisable sampling} and assignment construct, combining sampling from the standard normal and diffeomorphic transformations.}

\subsection{Syntax and Operational (Value) Semantics}
\label{sec:ops}
We fix \emph{latent variables} $z_1,\ldots,z_m$ and \emph{program variables} typically denoted by $x$ \dw{or $v_1,\ldots$ better?}. % and $z_i$ are the latent variables w.r.t. which the expectation is taken.
\emph{Expressions} and \emph{programs} are defined inductively as
\begin{align*}
  E&::= z_j\mid x\mid r\mid E+E\mid E\cdot E\mid -E\\
  P&::= \skipp\mid P;P\mid x:= E\\
  &\mid x:=\ifc EEE\\
  &\mid z_j\sim\dist(E,\ldots,E)\mid\observe E {\dist(E,\ldots,E)}
\end{align*}
where $r\in\Real$ is a real constant.

\iffalse
\lo{or, more pedantically, $\phi_{({-})}{({-})}:\Real^m\times\Real^{\ell+1}\to\Real$}
\fi


\changed[dw]{A key requirement is that each $\alpha_j$ which is used must be bound before, and cannot be re-assigned in the same branch.}

\lo{This requirement is not very clear. Do you mean: every occurrence of $\alpha_j$ in an expression must be preceded (in the computation path) by a $\alpha_j$-assignment.}
\dw{Yes.}
\dw{details, type system, appendix}

Intuitively, the latter non-standard construct samples from the standard normal distribution and immediately applies a transformation.
In this way, for example, sampling from arbitrary normal distributions $\nd(\mu,\sigma)$ can be simulated by $\underline\phi_{\mu,\sigma}(\sample)$,
where $\underline\phi_{\mu,\sigma}(z)\defeq\sigma\cdot z+\mu$.

\lo{I assume that in this paper we do not underline syntactic objects right? So the underline of the preceding $\underline\phi_{\mu,\sigma}(\sample)$ (and in several other places) should now be removed?}

For $\phi_\theta(z)\defeq z+\theta$ the function in \cref{ex:biased} can be expressed as the value returned by the following term when substituting $z$ as the sample:
\begin{align*}
  &\alpha:=\phi_\theta(\sample);\\
  &\ifc\alpha{-0.5\cdot\theta\cdot\theta}{1-0.5\cdot\theta\cdot\theta}
\end{align*}

\subsection{Semantics}
In the spirit of \cite{K79,BLGS16}, we view a probabilistic program as a deterministic function mapping parameters and \emph{traces} (which are sequences of random samples) to values.

Formally, we can endow the language with a (denotational) semantics, keeping track of the trace of random samples \cite{BLGS16,MOPW}.

An \emph{assignment} (typically $\ass$) is a partial function from variables to $\Real$. Expressions $E$ are interpreted in a standard way as $\sem  E(\ass)$ \dw{perhaps in appendix}. Given an assignment $\ass$ and a trace of random samples $\tr$, we can interpret a program (deterministically) as $\sem P(\ass,\tr)$, which is defined in \cref{fig:sem}. \dw{notation}
\begin{figure*}
  \begin{align*}
    \sem \skipp(\tr,\ass,w) &= (\tr,\ass, w)\\
    \sem{P;Q}(\tr,\ass,w)&\defeq \sem Q(\tr,\sem P(,\tr,\ass,w))\\
    \sem {x:=E}(\tr,\ass,w)&\defeq (\ass[x\mapsto\sem E(\ass)],w)\\
    \sem{\ifc EPQ}(\tr,\ass,w)&\defeq
    \begin{cases}
      \sem P(\tr,\ass,w)&\tif\sem E(\ass)<0\\
      \sem Q(\tr,\ass,w)&\tow
    \end{cases}\\
    \sem{z_j\sim\dist(E_1,\ldots,E_\ell)}(\tr,\ass,w)&\defeq(\ass[z_j\mapsto s_j],\pdf_{\dist(\sem{E_1}(\ass),\ldots,\sem{E_\ell}(\ass))}(s_j))\\
    \sem{\observe E{\dist(E_1,\ldots,E_\ell)}}(\tr,\ass,w)&\defeq(\ass,\pdf_{\dist(\sem{E_1}(\ass),\ldots,\sem{E_\ell}(\ass))}(\sem E(\ass)))
  %   \\
  %   \sem E(\ass,\tr)&\defeq\sem E(\ass)\\
  % \sem {\alpha_j:= \underline\phi_\para(E_1,\ldots,E_\ell,\sample);P}(\ass,\tr)&\defeq\sem P(\ass[\alpha_j\mapsto\phi_\para(\sem {E_1}(\ass),\ldots,\sem {E_\ell}(\ass),s_j)])\\
  % \sem{\ifc E PQ}(\ass,\tr)&\defeq
  % \begin{cases}
  %   \sem P(\ass,\tr)&\tif\sem E(\ass)<0\\
  %   \sem Q(\ass,\tr)&\tow
  % \end{cases}
  \end{align*}
  \caption{Semantics of Programs}
  \label{fig:sem}
\end{figure*}
\dw{Intuition?}
We are mainly concerned with programs where all $\alpha_j$ occur bound. Therefore, we abuse notation and write $\sem P(\para,\lat)$ for $\sem P(\rho,\tr)$, where $\rho(\theta_i)\defeq\theta_i$ and $s_j\defeq z_j$.
\lo{$\rho(\theta_i)\defeq\theta_i$ is confusing: $\rho$ is defined to be a map from variables to reals. So it follows from $\rho(\theta_i)\defeq\theta_i$ that the variable $\theta_i$ and the real $\theta_i$ are same?}

% In particular, for all $s\in\Real$ (the samples)
% % \dw{NB. simplified setting} \lo{Good!}%\dw{simplify here for when $M_i$ don't sample, or to $\ell=0$?}
% \begin{align*}
%   \underline\phi_\para(\sample)\Downarrow^{(s)}\underline{\phi_\para(s)}
%   % \infer[s\in\Real]{\underline\phi_\para(M_1,\ldots,M_\ell,\sample)\Downarrow^{^{\mathbf{s^{(1)}}}\app\cdots\app^{\mathbf{s^{(\ell)}}}\app(s)}\underline{\phi_\para(r_1,\ldots,r_\ell,s)}}{M_1\Downarrow^{\mathbf{s^{(1)}}}\underline{r_1}&\cdots&M_\ell\Downarrow^{\mathbf{s^{(\ell)}}}\underline{r_\ell}}\\[10pt]
% \end{align*}
% % \dw{more details?}
% meaning, intuitively, that on trace $s$, the reparameterisable sampling construct $\underline\phi_\para(\sample)$ evaluates to the numeral $\underline{\phi_\para(s)}$.
% \dw{adapt} Note that %due to the fact that
% because our language does not have recursion/iteration there is a bound $n\in\nat$ on the number of samples drawn on each path.
% Therefore, for all \changed[dw]{terms $M$ of type $\PCFReal$}, values $r_1,\ldots,r_m\in\Real$ (for the parameters $\theta_1,\ldots,\theta_m$) and samples $s_1,\ldots,s_n\in\Real$,
% there exists a unique prefix s.t.\ $M[r_1/\theta_1,\ldots,r_m/\theta_m]\Downarrow^{(s_1,\ldots,s_\ell)}\underline {r}$;
% and we write $\sem M((r_1,\ldots,r_n),(s_1,\ldots,s_n))=r$ in that case.
In probabilistic programming, this function
\begin{align*}
  \sem P\from\Real^m\times\Real^n\to\Real
\end{align*}
 is called the \emph{value function} of $P$ \cite{BLGS16}. \dw{NB this is quite dense}

% Henceforth, %we do not distinguish between the (formal) parameters and their instances (real numbers),
% we do not distinguish between the \emph{formal} parameters (variables) and the \emph{actual} parameters (real numbers),
% % \lo{These are their technical names in PL.}
% and we write $\sem M(\para,\lat)$ all the same, by abuse of notation.

Also note, that in the present work, because of the absence of a conditioning / score construct in our language, we are not explicitly concerned with the accompanying \emph{weight} (or \emph{density}) function (see \cite{BLGS16} for more details).
% \lo{A very apt addition, this!}
\dw{Tim suggests omiting this.} \lo{If we are short of space, this paragraph can go.}









We can phrase our optimisation problem as:

\begin{center}
\noindent\begin{fminipage}{.95\columnwidth}
\[
%\begin{align*}
  \text{argmin}_\para \ \E_{\lat\sim\msnd}[\sem P(\para,\lat)] \tag{\text{\textbf{P}}}\label{eq:optp}
%\end{align*}
%\label{eq:opt problem}
\]
where $\sem P:\Real^m\times\Real^n\to\Real$ is the value-function of a program $P$ and $\msnd$ is the multivariate standard normal distribution.
\end{fminipage}
\end{center}
For simplicity's sake we focus on expectations w.r.t.~normal distributions in this work.

\subsection{Translation to Smoothed Programs}
% Smoothed Programs (typically denoted by $P_\eta$) do not contain conditional assignements but may contain

\section{A Well-Behaved Class of Discontinuous Functions}
\dw{better section title}

Since (only) piecewise polynomials are expressible in our language and (absolute) moments of normals are finite (cf.~\cref{lem:punib}) we obtain:
\begin{proposition}[Integrability]
  For every $\para\in\Real^m$,
  \begin{align*}
    \E_{\lat\sim\msnd}[|\sem M(\para,\lat)|]<\infty
  \end{align*}
\end{proposition}
Therefore, the optimisation problem \eqref{eq:optp} \dw{\eqref{eq:info}} is well-defined.

%\paragraph{Discussion.}
\begin{remark}
\label{rem:adv of polys}
%\lo{Changed from Discussion to Remark - more standard and easier to reference.}
As stated initially, we are mainly motivated by variational inference.
If we restrict ourselves to normal distributions,
each branch of the densities $p$ and $q_\para$ \lo{I assume you refer to the $p$ and $q_\para$ in line 023?} are the product of normal densities, the logarithm of which are (bounded by) polynomials.
In particular, the counterexample in \citep[Proposition~2]{LYY18} is of this form.

The main advantage is that polynomials have pleasing (closure) properties.
Note that permitting exponential functions injudiciously may render the optimisation problem \eqref{eq:optp} ill-defined,
for example, $\E_{z\sim\nd(0,1)}[\exp(z^2)]=\infty$ (independent of parameters).
%\lo{Strictly speaking, this is a feasibility problem (which asks: is the feasible / solution set empty?), not optimisation, though it is a prior problem and so highly relevant to optimisation, of course.}
\end{remark}

\subsection{PPRPP}
% We aim to ensure that the value functions of terms of type $\PCFReal$ are finite sums of functions $\Real^m\times\Real^n\to\Real$ of the form

\dw{check when compactness becomes necessary}
\changed[dw]{Henceforth we fix a set $\parasp\subseteq\Real^m$. A \emph{piecewise polynomial under reparametrised polynomial partitions (PPRPP)} is a finite sum of functions $\Real^m\times\Real^n\to\Real$ of the form
}
\begin{align}
%  \Real^m\times\Real^n&\to\Real\nonumber\\
  (\para,\lat)&\mapsto
  \begin{cases}
    p(\para,\lat)&\tif \text{for all $\psi\in\bpl$, $\psi(\rep_\para(\lat))<0$,}\\
    &\text{and for all $\psi\in\bpgeq$, $\psi(\rep_\para(\lat))\geq 0$}\\
    0&\tow
  \end{cases}
  \label{eq:form}
\end{align}
where
\begin{enumerate}[label=(V\arabic*),leftmargin=32pt]
  \item\label{it:const} $\bpl$ and $\bpgeq$ are finite sets of polynomials $\Real^n\to\Real$ \changed[dw]{which are not constant\footnote{This will be used in the uniform convergence proofs (cf.~\cref{prop:unifg,lem:sigsim}).} $0$}
  \item\label{it:diffeo}
  \changed[dw]{  $\inf_{(\para,\lat)\in\parasp\times\Real^n}|\det\Jac_\lat\rep_\para(\lat)|>0$.
} \dw{does this work in measure}
  % $\rep_\para=\langle\phi_\para^{(1)},\ldots,\phi_\para^{(n)}\rangle\from\Real^n\to\Real^n$ for strong diffeomorphisms (cf.~\cref{eq:strdiff}) $\phi^{(i)}_\para\from\Real^i\to\Real$. \dw{lifted}
  \item\label{it:poly} $p\from\Real^m\times\Real^n\to\Real$ is a polynomial.
\end{enumerate}
Intuitively, $\bpl$ and $\bpgeq$ correspond to the constraints imposed by the if-branching, and $\rep_\para$ is the transformation in a branch.

\changed[dw]{In particular, every affine transformation is a strong diffeomorphism\footnote{A (contrived) counterexample is $\phi(z_1,z_2)\defeq z_1^2z_2+\frac 1 3 z_1^2 z_2^3-z_1z_2^2+z_2$ because $\frac{\partial\phi}{\partial z_2}(z_1,z_2)=z_1^2+(z_1z_2-1)^2$ has no positive lower bound despite being everywhere positive.}.
} \lo{Strong diffeomorphism is not defined yet.}

\changed[dw]{An important consequence of this is that within a branch of computation (corresponding to a summand (of the form~(\ref{eq:form})) all guards only depend on transformed variables, and they are obtained by the same diffeomorphism.
This will allow us to cast partial derivatives w.r.t.\ a parameter $\theta$ in terms of gradients w.r.t.\ the noise variables $\lat$ (see \cref{eq:extrick}).}



\begin{remark}
\label{rem:type system}
In particular, these conditions rule out optimisation problems whose objective functions are \emph{discontinuous} such as\footnote{Given predicate $\psi$, we write $[\psi]$ as the Iverson bracket.}
\changed[dw]{
\begin{equation*}
\E_{z\sim\nd(0,1)}[\sem{\alpha:=\sample;\ifc\theta{ 0}{ 1}}(\theta,z)]=[\theta\geq 0]
% \label{eq:discts obj fn}
\end{equation*}
}
% \lo{Added round brackets above.}
% \dw{What is the purpose of the round brackets? I've never seen a notation like this.}
% \lo{Sorry - I placed the brackets at the wrong place.
% I have now removed them altogether.
% I just wanted to clarify the parsing. I.e.\ the intended objective function is an equation, rather than an expectation. I.e.\ it is \emph{not}
% \[
% \E_{z\sim\nd(0,1)}\Big[\big(\ifc\theta{\underline 0}{\underline 1}\big)=[\theta\geq 0]\Big]
% \]
% }
% \dw{I'd think that ``feasibility'' may be confusing here since the paper isn't concerned with it.}
% \lo{On second thought, \cref{eq:discts obj fn} still makes sense as an objective function for an optimisation problem.
% So I will drop any mention of feasibility problem.}
%\lo{This is a feasibility problem (i.e.~determine / characterise the solution set, rather than identify stationary points), rather than optimisation of a cost.}
where the expectation itself is discontinuous, rather than just the function inside the expectation.

Though important (in our view), it is unfortunate that general discontinuous \emph{and} non-convex optimisation does not appear to have attracted much attention (in the machine learning community) with the notable exception of \cite{MoreauA00,Z81,BagirovKM14,BagirovGKMT20}. %\dw{reference?} \lo{Should perhaps also cite \cite{BagirovKM14} and \cite{BagirovGKMT20} and work of their school.}
\end{remark}





\subsection{Restrictions to the PL}
\label{sec:type}
In order to ensure that programs denote PPRPPs we impose two minor restrictions:
\begin{enumerate}
  \item Each $\rep_\para:\Real^m\times\Real^{\ell}\to\Real$ is a \emph{strong diffeomorphism}:
  \begin{align}
    \label{eq:strdiff}
    \inf_{\para\in\parasp}\inf_{z_1,\ldots,z_\ell\in\Real}\left|\frac{\partial\phi_\para}{\partial z_\ell}(z_1,\ldots,z_\ell)\right|>0
  \end{align}
\item In branching subprograms $\ifc EPQ$ the guard $E$ does not contain parameters $\theta_i$ (but it may contain variables $\alpha_j$, which may depend \lo{(via a $\alpha_j$-assignment)} on the parameter through a transformation).
\end{enumerate}




Thus, our type system needs to enforce the constraint that guards do not directly depend on parameters $\theta_i$ (but, possibly, only indirectly through transformations).
In particular,
\begin{gather*}
  \ifc\theta 0 1\\
  x:=\theta; \ifc{x} 0 1
\end{gather*}
are not typable, but the following terms are typable
\begin{gather*}
  x:= \underline\phi_\theta(\sample);\ifc{x} 0 1\\
  x:= \underline\phi_\theta(\sample);
  \ifc x{\underline{-0.5}\cdot\theta^2}{\underline{-0.5}\cdot\theta^2+\underline 1})
\end{gather*}
although for each sampled value the parameter $\theta$ may influence which branch is taken.
Note that for $\phi_\theta(z)\defeq z+\theta$ the value-function of the latter term corresponds to \cref{ex:biased}.

\lo{Typo in the following?}

$\sem P\Real^m\times\Real^{j}\times\Real^{n-j}\to\Real$


\begin{lemma}
  $\sem E$ is a polynomial
\end{lemma}

\begin{restatable}{lemma}{PLres}
  Under these restrictions $\sem P$ is PPRPP.
\end{restatable}

$\Gamma\vdash_e E$
\begin{gather*}
  \infer[\alpha_j\not\in\Gamma]{\Gamma\vdash\alpha_j:=\phi_\para(E_1,\ldots,E_\ell,\sample);P}{\Gamma\vdash_e E_1&\ldots&\Gamma\vdash_e E_\ell&\Gamma,\alpha_j\vdash P}\\
  \infer{\Gamma\vdash\ifc E PQ}{\Gamma\setminus\para\vdash_e E&\Gamma\vdash P&\Gamma\vdash Q}
\end{gather*}



\newcommand\vars{\mathrm{Vars}}
\newcommand\exps{E_{\mathrm{strict}}}
\newcommand\varss{\vars_{\mathrm{strict}}}

\section{Extending the PL}
We assume $\varss,\{\theta_1,\ldots,\theta_n\}\subseteq\vars$ and $\varss$ does not contain any $\theta_i$.


\newcommand\xs{x_{\mathrm{strict}}}
\changed[dw]{Define expressions, instructions and programs, respectively:}
\begin{align*}
  \exps &::=\xs\mid\underline r\mid\exps+\exps\mid\exps\cdot\exps\\
  &\mid\underline\phi_\para(E,\ldots,E,\sample)\\
  E&::=\exps\mid x\mid E+E\mid E\cdot E\\
  M&::=  \xs := \exps\mid x:=E \mid \{M;M\}\\
  P&::= E \mid M; P\mid\ifc {\exps} PP\\
  &\mid \ifc\exps MM;P
  %  &\mid\underline\phi_\para(M,\ldots,M,\sample)
\end{align*}
where $\xs\in\varss$ and $x\in\vars$.

\begin{enumerate}
  \item Replace subexpressions $\underline\phi_\para(E,\ldots,E,\sample)$  with fresh variable $\alpha\in\varss$ and add assignment $\alpha:=\underline\phi_\para(E,\ldots,E,\sample)$.
  \item Remove $\ifc\exps MN;P$ by $\ifc\exps{M;P}{N;P}$.
  \item In each branch, if last instruction is assignment $x:= E$ replace with $E$.
  \item Remove deterministic assignments by substituting assigned terms
\end{enumerate}

\begin{example}
  We start with
  \begin{align*}
&\ifc {\phi_\theta(\sample)}{y:=0}{y:=1};\\
&res:=-0.5\cdot \theta\cdot\theta + y
  \end{align*}
  is transformed to
  \begin{align*}
    &\alpha:=\phi_\theta(\sample)\\
    &\ifc\alpha{-0.5\cdot\theta\cdot\theta + 0}{-0.5\cdot\theta\cdot\theta + 1}
  \end{align*}

  \iffalse
  \begin{lstlisting}
  if (*$\phi_\theta$*)(sample) < 0 then y:=0 else y:=1;
  res := -0.5*(*$\theta$*)*(*$\theta$*) + y
  \end{lstlisting}
  Step 1:
  \begin{lstlisting}
  (*$\alpha$*) := (*$\phi_\theta$*)(sample)
  if (*$\alpha$*) < 0 then y:=0 else y:=1;
  res := -0.5*(*$\theta$*)*(*$\theta$*) + y
  \end{lstlisting}
  Step 2:
  \begin{lstlisting}
  (*$\alpha$*) := (*$\phi_\theta$*)(sample)
  if (*$\alpha$*) < 0 then
    {y:=0; res := -0.5*(*$\theta$*)*(*$\theta$*) + y}
  else
    {y:=1; res := -0.5*(*$\theta$*)*(*$\theta$*) + y}
  \end{lstlisting}
  Step 3:
  \begin{lstlisting}
  (*$\alpha$*) := (*$\phi_\theta$*)(sample)
  if (*$\alpha$*) < 0 then
    {y:=0; -0.5*(*$\theta$*)*(*$\theta$*) + y}
  else
    {y:=1; -0.5*(*$\theta$*)*(*$\theta$*) + y}
  \end{lstlisting}
  Step 4:
  \begin{lstlisting}
  (*$\alpha$*) := (*$\phi_\theta$*)(sample)
  if (*$\alpha$*) < 0 then
    -0.5*(*$\theta$*)*(*$\theta$*) + 0
  else
    -0.5*(*$\theta$*)*(*$\theta$*) + 1
  \end{lstlisting}
  \fi
\end{example}


\section{Supplementary Materials for \cref{sec:pl}}
\label{app:pl}

\PLres*
\begin{proof}
  W.l.o.g.\ we assume that in subprograms $\alpha_j:=\phi_\para(E,\ldots,E,\sample);P$ only variables amongst $\alpha_{j+1},\ldots,\alpha_n$ are bound.

  We prove the following stronger claim:
  Suppose $\Gamma\vdash P$ and for $\alpha_j\in\Gamma$, $\phi^{(j)}_\para:\Real^j\to\Real$ is a polynomial satisfying
  \begin{align}
    \label{eq:repb}
    \inf_{\para\in\parasp}\inf_{s_1,\ldots,s_j\in\Real}\left|\frac{\partial\phi_\para^{(j)}}{\partial s_j}(s_1,\ldots,s_j)\right|>0
  \end{align}
Then $(\para,\tr)\mapsto\sem P(\rho_{\para,\tr},\tr)$ is a PPRPP
 \begin{align*}
   \sem P(\ass_{\para,\tr},\tr)&=\sum_{i=1}^\ell p^{(i)}(\para,\tr)\cdot\prod_{\psi\in\Psi_<^{(i)}} [\psi(\rep_\para^{(i)}(\para,\tr))<0]\cdot\prod_{\psi\in\Psi_\geq^{(i)}} [\psi(\rep_\para^{(i)}(\para,\tr))\geq 0]
 \end{align*}
 where
   $\ass_{\para,\tr}(\alpha_j)\defeq\phi_\para^{(j)}(s_1,\ldots,s_j)$.

   \dw{This is confusing/wrong notation-wise.}

  %  such that
  % such that
  % \begin{align}
  %   \label{eq:repvar}
  %   \rep_\para^{(i)}(\tr)_k=\ass_{\para,\tr}(\alpha_k)
  % \end{align} for $\alpha_k\in\Gamma$. \dw{notation}


  First, note that for programs which are expressions $E$ this is immediate because $\rho_{\para,\tr}$ is polynomial.

  First, suppose $\alpha_j:=\phi_\para^{(j)}(E_1,\ldots,E_\ell,\sample);P$.
  Let $\ass'_{\para,\tr}\defeq[\alpha_j\mapsto\phi_\para^{(j)}(\sem {E_1}(\ass_{\para,\tr}),\ldots,\sem {E_{\ell}}(\ass_{\para,\tr}),s_j)]$. Since $\alpha_j$ does not occur in the $E_i$, by the chain rule
  \begin{align*}
    \frac{\partial \ass'_{\para,\tr}}{\partial s_j}(\alpha_j)=\frac{\partial\phi_\para^{(j)}}{\partial x_{\ell+1}}(\sem {E_1}(\ass_{\para,\tr}),\ldots,\sem {E_{\ell}}(\ass_{\para,\tr}),s_j)
  \end{align*}
  Since $\phi_\para^{(j)}$ is assumed to be a strong diffeomorphism the inductive hypothesis is applicable to $P$ and $\ass'_{\para,\tr}$.
   The claim follows because $\sem{\alpha_k:=\phi_\para^{(k)}(E_1,\ldots,E_\ell,\sample);P}(\ass_{\para,\tr},\tr)=\sem P(\ass'_{\para,\tr},\tr)$.

  Next, suppose $\ifc E PQ$.
If $\sem E=0$ then $\sem{\ifc E PQ}=\sem Q$ and the claim follows from the inductive hypothesis.
 Otherwise by the inductive hypothesis there exists,
  \begin{align*}
    \sem P(\ass_{\para,\tr},\tr)&=\sum_{i=1}^\ell p^{(i)}(\para,\tr)\cdot\prod_{\psi\in\Psi_<^{(i)}} [\psi(\rep_\para^{(i)}(\para,\tr))<0]\cdot\prod_{\psi\in\Psi_\geq^{(i)}} [\psi(\rep_\para^{(i)}(\para,\tr))\geq 0]\\
    \sem Q(\ass_{\para,\tr},\tr)&=\sum_{j=1}^{\widehat\ell} q^{(i)}(\para,\tr)\cdot\prod_{\psi\in\widehat\Psi_<^{(j)}} [\psi(\widehat\rep_\para^{(j)}(\para,\tr))<0]\cdot\prod_{\psi\in\widehat\Psi_\geq^{(j)}} [\psi(\widehat\rep_\para^{(j)}(\para,\tr))\geq 0]
  \end{align*}
    Note that $\Gamma\setminus\para\vdash_e E$. Therefore, $\sem E$ does not depend on the parameters $\para$ and is a polynomial. Thus, by \cref{eq:repvar} there exists a polynomial $\chi:\Real^n\to\Real$ which is not constant $0$ such that %$\sem E(\ass_{\para,\tr})=p(\rep)$
    $\sem E(\ass_{\para,\tr})=\chi(\rep^{(i)}_\para(\tr))=\chi(\widehat\rep^{(j)}_\para(\tr))$.

  Therefore,
  \begin{align*}
    \sem{\ifc EPQ}(\ass_{\para,\tr},\tr)&=[\sem E(\ass_{\para,\tr},\tr)<0]\cdot\sem P(\ass_{\para,\tr},\tr)+[\sem E(\ass_{\para,\tr},\tr)\geq 0]\cdot\sem Q(\ass_{\para,\tr},\tr)\\
    &=\sum_{i=1}^\ell p^{(i)}(\para,\tr)\cdot\left[\chi(\rep_\para^{(i)}(\para,\tr))<0\right]\prod_{\psi\in\Psi_<^{(i)}} [\psi(\rep_\para^{(i)}(\para,\tr))<0]\cdot\prod_{\psi\in\Psi_\geq^{(i)}} [\psi(\rep_\para^{(i)}(\para,\tr))\geq 0]\\
    &+\sum_{j=1}^{\widehat\ell} q^{(i)}(\para,\tr)\cdot\prod_{\psi\in\widehat\Psi_<^{(j)}} [\psi(\widehat\rep_\para^{(j)}(\para,\tr))<0]\cdot\left[\chi(\widehat\rep_\para^{(j)}(\para,\tr))\geq 0\right]\cdot\prod_{\psi\in\widehat\Psi_\geq^{(j)}} [\psi(\widehat\rep_\para^{(j)}(\para,\tr))\geq 0]
  \end{align*}
\end{proof}




\section{Supplementary Materials for \cref{sec:IUC}}
\label{app:IUC}
We focus on the following setting. The results of \cref{sec:IUC} will follow by linearity.
\changed[dw]{
\begin{assumption}
  \label{ass:ass}
  \begin{enumerate}
    \item $\parasp\subseteq\Real^m$ is compact.
    \item $p:\Real^m\times\Real^n\to\Real$ and $\psi_1,\ldots,\psi_\ell\from\Real^n\to\Real$ are polynomials and the $\psi_i$ are not constant $0$.
    \item\label{ass:diff} For $j\in\{1,\ldots,n\}$, $\phi^{(j)}_{\para}\from\Real^j\to\Real^n$ is a diffeomorphic polynomial such that
    $\inf_{\para\in\parasp}\inf_{z_1,\ldots,z_j\in\Real}\left|\frac{\partial\phi^{(j)}}{\partial z_j}(\para,(z_1,\ldots,z_j))\right|> 0$
  \end{enumerate}
\end{assumption}}
\dw{NB: strengthened}
Define
\begin{align*}
  \Psi(\repx)&\defeq \prod_{i=1}^{\ell'}[\psi_i(\repx)\geq 0]\cdot\prod_{i=\ell'+1}^\ell[\psi_i(\repx)>0]&\Psi_k(\repx)&\defeq \prod_{i=1}^\ell\sigma_k(\psi_i(\repx))\\
  \rep_\para(\lat)&\defeq\left\langle\phi_\para^{(1)}(z_1),\ldots,\phi_\para^{(n)}(z_1,\ldots,z_n)\right\rangle\\
  f(\para,\lat)&\defeq p(\para,\lat)\cdot\Psi(\rep_\para(\lat))&
  f_k(\para,\lat)&\defeq p(\para,\lat)\cdot\Psi_k(\rep_\para(\lat))
\end{align*}

\subsection{Supplementary Materials for \cref{sec:unb}}
\label{app:unb}

The following immediately follows from a well-known result about exchanging differentiation and integration, which is a consequence of the dominated convergence theorem \citep[Theorem 6.28]{K13}:
\begin{lemma}
  \label{lem:meas}
  Let $U \subseteq\Real$ be \changed[dw]{open}. Suppose $g\from\Real\times\Real^n\to\Real$ satisfies
  \begin{enumerate}
    \item for each $x\in\Real$, $\lat\mapsto g(x,\lat)$ is integrable
    \item $g$ is continuously differentiable everywhere
    \item there exists integrable $h\from\Real^n\to\Real$ such that for all $x\in U$ and $\lat\in\Real^n$, $|\frac{\partial g}{\partial x}(x,\lat)|\leq h(\lat)$.
  \end{enumerate}
  Then for all $x\in U$, $\frac\partial{\partial x}\int g(x,\lat)\diff\lat=\int\frac{\partial g}{\partial x}(x,\lat)\diff\lat$.
\end{lemma}

\begin{corollary}
  \label{cor:meas}
  Let $i\in\{1,\ldots,m\}$, $M>0$ and $U\defeq B_M(\mathbf 0)\subseteq\Real^m$ be the \changed[dw]{open $M$-ball}. Suppose $g\from\Real^m\times\Real^n\to\Real$ satisfies
  \begin{enumerate}
    \item for each $\mathbf x\in\Real^m$, $\lat\mapsto g(\mathbf x,\lat)$ is integrable
    \item $g$ is continuously differentiable everywhere
    \item there exists integrable $h\from\Real^n\to\Real$ such that for all $\mathbf x\in U$ and $\lat\in\Real^n$, $|\frac{\partial g}{\partial x_i}(\mathbf x,\lat)|\leq h(\lat)$.
  \end{enumerate}
  Then for all $\mathbf x\in U$, $\frac\partial{\partial x_i}\int g(\mathbf x,\lat)\diff\lat=\int\frac{\partial g}{\partial x_i}(\mathbf x,\lat)\diff\lat$.
\end{corollary}

\begin{proposition}
  \label{prop:unbaux}
%  \label{prop:expdiff}
  For all $k\in\nat$, $\para\in\Real^m$ and $i\in\{1,\ldots,m\}$,
  \begin{align*}
    \frac\partial{\partial\theta_i}\E_\lat\left[f_k(\para,\lat)\right]=\E_\lat\left[\frac{\partial}{\partial\theta_i}f_k(\para,\lat)\right]
  \end{align*}
  % \begin{align*}
  %   \frac\partial{\partial\theta_j}\E_\lat\left[p(\para,\lat)\cdot\prod_{i=1}^\ell\sigma_k(p_i(\para,\lat))\right]=\E_\lat\left[\frac{\partial}{\partial\theta_j}\left(p(\para,\lat)\cdot\prod_{i=1}^\ell\sigma_k(p_i(\para,\lat))\right)\right]
  % \end{align*}
\end{proposition}
\begin{proof}
  Suppose $k\in\nat$, $\para\in\Real^m$ and $i\in\{1,\ldots,m\}$. Clearly, there exists $M>0$ such that $\para\in B_M(\mathbf 0)\subseteq\Real^m$.

  For $j\in\{1,\ldots,\ell\}$, abbreviate $p_j(\para,\lat)\defeq\psi_j(\rep_\para(\lat))$, which are polynomials.
%  Suppose $k\in\nat$, $\para\in\parasp$ and $j\in\{1,\ldots,m\}$. Then
Note
  \begin{align*}
    &\left|\frac{\partial}{\partial\theta_i}\left(p(\para,\lat)\cdot\prod_{j=1}^\ell\sigma_k(p_j(\para,\lat))\right)\right|\\
    &\leq\left|\frac{\partial p}{\partial\theta_i}(\para,\lat)\right|+\left|p(\para,\lat)\cdot\sum_{j=1}^\ell\sigma_k'(p_j(\para,\lat))\cdot\frac{\partial p_j}{\partial\theta_i}(\para,\lat)\cdot\prod_{j'\neq j}\sigma(p_{j'}(\para,\lat)) \right|\\
    &\leq\left|\frac{\partial p}{\partial\theta_i}(\para,\lat)\right|+\left|p(\para,\lat)\cdot\sum_{j=1}^\ell\frac{\sqrt k} 4\cdot\frac{\partial p_j}{\partial\theta_i}(\para,\lat) \right|\\
    &\leq\left|\underbrace{\frac{\partial p}{\partial\theta_i}(\para,\lat)}_{\text{polynomial}}\right|+\frac{\sqrt k} 4\cdot\sum_{j=1}^\ell\left|\underbrace{p(\para,\lat)\cdot\frac{\partial p_j}{\partial\theta_i}(\para,\lat)}_{\text{polynomial}} \right|
  \end{align*}
  because $\sigma_k'\leq\frac{\sqrt k}4$.
  By \cref{lem:puniq}  the summands can be uniformly bounded on the closure of $B_M(\mathbf 0)$ by the absolute value of an (integrable) polynomial. The claim follows by \cref{cor:meas}.
\end{proof}

\cref{prop:unb} follows by linearity.


\subsection{Supplementary Materials for \cref{sec:unic}}
\changed[dw]{Note that by \cref{ass:diff} of \cref{ass:ass}, $\Jac_\lat\rep_\para(\lat)$ is (lower) triangular and invertible. In particular,
\begin{lemma}
  \label{lem:lbdet}
  There exists %$L>0$
  $M>0$ such that $|\det\Jac_\lat\rep_\para(\lat)|>M$ for all $\para\in\parasp$ and $\lat\in\Real^n$.
\end{lemma}}
% \begin{proof}
%   By the assumption for every $\para\in\parasp$
%   £££
%   Note that
%   $(\para,\lat)\mapsto\det\left(\Jac_\lat\rep_\para(\lat)\right)$
%   is a polynomial (in particular continuous). Besides, since each $\rep_\para$ is a diffeomorphism, $\det(\Jac_\lat\rep(\para,\lat))\neq 0$ for all $\para$ and $\lat$.
%   \dw{Details: for each $\para\in\parasp$ by continuity of $\lat\mapsto\det\left(\Jac_\lat\rep_\para(\lat)\right)$, $\inf_\lat \det\left(\Jac_\lat\rep_\para(\lat)\right)=:M_\para >0$ (it's a polynomial, so goes to $\pm\infty$). By compactness of $\parasp$, $M\defeq\min_{\para\in\parasp} M_\para>0$.}
% \end{proof}

Hence,
\begin{align*}
  \vel_i\from\Real^m\times\Real^n&\to\Real^n\\
  (\para,\lat)&\mapsto \Jac^{-1}_\lat \rep_\para(\lat)\cdot\Jac_{\theta_i} \rep_\para(\lat)
\end{align*}
 is well-defined.

As a consequence, we can express partial derivatives w.r.t.\ a parameter $\theta_i$ in terms of the gradient w.r.t.\ the latent variables $\lat$.
\begin{align}
  \frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial\theta_i}(\para,\lat)%&=\nabla_\lat(\Psi_k\circ\rep_{(-)})(\para,\lat)\cdot\Jac_\lat^{-1}\rep_\para(\lat)\cdot\Jac_{\theta_i}\rep_\para(\lat)\nonumber\\
   &=
  \nabla\Psi_k(\rep_\para(\lat))\cdot\Jac_{\theta_i}\rep_\para(\lat)\notag\\
  \intertext{(Here it is crucial that the guards, i.e.\ the $\psi_i$ in the definition of $\Psi_k$, do not depend on the parameters $\para$.)}
  &=\nabla\Psi_k(\rep_\para(\lat))\cdot\Jac_\lat\rep_\para(\lat)\cdot(\Jac_\lat\rep_\para(\lat))^{-1}\cdot\Jac_{\theta_i}\rep_\para(\lat)\notag\\
  &=\nabla_\lat(\Psi_k\circ\rep_{(-)}(-))(\para,\lat)\cdot \Jac^{-1}_\lat\rep_\para(\lat))\cdot\Jac_{\theta_i}\rep_\para(\lat)\notag\\
  &=\nabla_\lat(\Psi_k\circ\rep_{(-)})(\para,\lat)\cdot\vel_i(\para,\lat)  \label{eq:trick}
\end{align}
Note that for this it is essential that the guards, i.e.\ the $\psi_i$ in the definition of $\Psi_k$, do not depend on the parameters $\para$, but that all $\psi_i$ are composed with the same transformation\footnote{in this particular branch of the computation} $\rep_\para$.

\begin{lemma}
  \label{lem:velbp}
  Let $i,i'\in\{1,\ldots m\}$ and $j,j'\in\{1,\ldots,n\}$.
  All of $|\vel_i|$, $|\frac{\partial\vel_i}{\partial z_j}|$, $|\frac{\partial^2\vel_i}{\partial\theta_{i'}\,\partial z_j}|$ and $|\frac{\partial^2\vel_i}{\partial z_j\,\partial z_{j'}}|$ are bounded by the absolute value of polynomials.
\end{lemma}
\begin{proof}
  Let $M>0$ as in \cref{lem:lbdet}.
  The claim for $\vel_i$ follows immediately from
  \begin{align*}
    \frac 1{\det(\Jac_\lat\rep(\para,\lat))}\leq\frac 1 M
  \end{align*}
  and the fact that adjugate (transpose of the cofactor matrix) is a polynomial. Similarly,
  \begin{align*}
    \left|\frac\partial{\partial z_j}\frac 1{\det(\Jac_\lat\rep_\para(\lat))}\right|&=
    \left|\frac 1{(\det(\Jac_\lat\rep_\para(\lat)))^2}\cdot\frac\partial{\partial z_j}\det(\Jac_\lat\rep_\para(\lat))\right|
    \leq\frac 1 {M^2}\cdot\left|\underbrace{\frac\partial{\partial z_j}\det(\Jac_\lat\rep_\para(\lat))}_{\text{polynomial}}\right|
  \end{align*}
  Similarly,
  \begin{align*}
    &\left|\frac{\partial^2}{\partial z_{j'}\,\partial z_j}\frac 1{\det(\Jac_\lat\rep_\para(\lat))}\right|\\
    &=\left|\frac\partial{\partial z_{j'}}\left(\frac 1{(\det(\Jac_\lat\rep_\para(\lat)))^2}\cdot\frac\partial{\partial z_j}\det(\Jac_\lat\rep_\para(\lat))\right)\right|\\
    &\leq\left|\frac 1{(\det(\Jac_\lat\rep_\para(\lat)))^2}\cdot\underbrace{\frac{\partial^2}{\partial z_{j'}\,\partial z_j}\det(\Jac_\lat\rep_\para(\lat))}_{\text{polynomial}}-\frac 2{(\det(\Jac_\lat\rep_\para(\lat)))^3}\cdot
    \underbrace{\frac\partial{\partial z_{j'}}\det(\Jac_\lat\rep_\para(\lat))\cdot
    \frac\partial{\partial z_j}\det(\Jac_\lat\rep_\para(\lat))}_{\text{polynomial}}\right|
  \end{align*}
  Similarly,
  \begin{align*}
    &\left|\frac{\partial^2}{\partial\theta_{i'}\,\partial z_j}\frac 1{\det(\Jac_\lat\rep_\para(\lat))}\right|\\
    &=\left|\frac\partial{\partial\theta_{i'}}\left(\frac 1{(\det(\Jac_\lat\rep_\para(\lat)))^2}\cdot\frac\partial{\partial z_j}\det(\Jac_\lat\rep_\para(\lat))\right)\right|\\
    &\leq\left|\frac 1{(\det(\Jac_\lat\rep_\para(\lat)))^2}\cdot\underbrace{\frac{\partial^2}{\partial\theta_{i'}\,\partial z_j}\det(\Jac_\lat\rep_\para(\lat))}_{\text{polynomial}}-\frac 2{(\det(\Jac_\lat\rep_\para(\lat)))^3}\cdot
    \underbrace{\frac\partial{\partial\theta_{i'}}\det(\Jac_\lat\rep_\para(\lat))\cdot
    \frac\partial{\partial z_j}\det(\Jac_\lat\rep_\para(\lat))}_{\text{polynomial}}\right|
  \end{align*}
\end{proof}

\iffalse
\begin{lemma}
Let $\ell\in\nat$.  There exists $L>0$ such that for all $\para\in\parasp$, $\E\left[\left|\frac\partial{\partial z_i}\frac 1{\det(\Jac_\lat\rep(\para,\lat))}\right|^\ell\right]<L$.
\end{lemma}
\begin{proof}
  \begin{align*}
    \E\left[\left|\frac\partial{\partial z_i}\frac 1{\det(\Jac_\lat\rep(\para,\lat))}\right|^\ell\right]&=
    \E\left[\left|\frac 1{(\det(\Jac_\lat\rep(\para,\lat)))^2}\right|^\ell\cdot\left|\frac\partial{\partial z_i}\det(\Jac_\lat\rep(\para,\lat))\right|^\ell\right]\\
    &\leq\E\left[\frac 1 {M^{2\ell}}\cdot\left|\frac\partial{\partial z_i}\det(\Jac_\lat\rep(\para,\lat))\right|^\ell\right]&\text{\cref{lem:lbdet}}\\
    &\leq\frac 1 {M^{2\ell}}\cdot\E\left[\left|\underbrace{\frac\partial{\partial z_i}\det(\Jac_\lat\rep(\para,\lat))}_{\text{polynomial}}\right|^\ell\right]
    % &\leq \E\left[\left|\frac 1{(\det(\Jac_\lat\rep(\para,\lat)))^2}\right|^{2\ell}\right]\cdot\E\left[\left|\frac\partial{\partial z_i}\underbrace{\det(\Jac_\lat\rep(\para,\lat))}_{\text{polynomial}}\right|^{2\ell}\right]\\
    % &\leq \E\left[\frac 1 {M^{4\ell}}\right]\cdot\E\left[\underbrace{\left|\frac\partial{\partial z_i}\det(\Jac_\lat\rep(\para,\lat))\right|^{2\ell}}_{\text{polynomial}}\right]\\
  \end{align*}
  and the claim follows from \cref{lem:punib}.
\end{proof}
Since the adjugate (transpose of the cofactor matrix) is polynomial we at once conclude employing \cref{lem:punib}:
\dw{is this what's needed?}
\begin{corollary}
  \label{cor:vbound}
  Let $\ell\in\nat$ and $i,j\in\{1,\ldots,n\}$. There exists $L>0$ such that for all $\para\in\parasp$, $\E\left[\left|\vel_{i,j}(\para,\lat)\right|^\ell\right]<L$ and $\E\left[\left|\frac\partial{\partial z_j}\vel_{i,j}(\para,\lat)\right|^\ell\right]<L$.
\end{corollary}

\dw{continue}


\begin{align*}
  \E_{\lat\sim\msnd}\left[\left|\frac{\partial(\Psi_k\circ\rep_\para)}{\partial\theta_i}(\lat)\right|^2\right]&\leq\sum_{j=1}^n\E_{\lat\sim\msnd}\left[\left|\frac{\partial}{\partial z_j}(\sigma_k\circ\Psi_k\circ\rep_{(-)})(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right|^2\right]\\
  &\leq\sum_{j=1}^n\sqrt{\E_{\lat\sim\msnd}\left[\left|\frac{\partial}{\partial z_j}(\sigma_k\circ\Psi_k\circ\rep_{(-)})(\para,\lat)\right|^4\right]\cdot\E_{\lat\sim\msnd}\left[\left|\vel_{i,j}(\para,\lat)\right|^4\right]}
\end{align*}

\fi


%Let $\mu$ be the standard normal probability measure.

\begin{lemma}
  \label{lem:sigsim}
  Let $0\neq q\from\Real^n\to\Real$ be a polynomial. There exist $L,\epsilon>0$ such that
  $\E_{\lat\sim\msnd}[|\sigma_{k+1}(q(\rep_\para(\lat)))-\sigma_k(q(\rep_\para(\lat)))|^2]< L\cdot k^{-2-\epsilon}$ for all $k\in\nat$ and $\para\in\parasp$.
\end{lemma}
\begin{proof}
  Let $0<\epsilon<\frac 1 2$.

  Let $K,L,\delta>0$ as in \cref{cor:polyr}.
  Suppose $k\in\nat$ and $\para\in\parasp$.
  By \cref{cor:polyr}, there exists $U\subseteq\Real^n$ such that $\E_{\lat\sim\msnd}[[\lat\in\rep_\para^{-1}( U)]]\leq K\cdot k^{-\delta}$ and for each $\repx\in\Real^n\setminus\rep_\para^{-1}( U)$, $|q(\repx)|>L\cdot k^{-\epsilon}$.
  Thus,
  \begin{align*}
    &\E_{\lat\sim\msnd}\left[\left|\sigma_{k+1}(q_\para(\lat))-\sigma_k(q_\para(\lat))\right|^2\right]\\
    &\leq\E_\lat\left[[\rep_\para(\lat)\in U]\cdot\left|\sigma_{k+1}(q_\para(\lat))-\sigma_k(q_\para(\lat))\right|^2\right]+\E_\lat\left[[\rep_\para(\lat)\in\Real^n\setminus U]\cdot\left|\sigma_{k+1}(q_\para(\lat))-\sigma_k(q_\para(\lat))\right|^2\right]\\
    &\leq\E_\lat\left[[\rep_\para(\lat)\in U]\cdot\frac 1 {k^2}\right]+\E_\lat\left[[\rep_\para(\lat)\in\Real^n\setminus U]\cdot\left|\frac 1 L\cdot k^{-\frac 3 2+\epsilon}\right|^2\right] \qquad \text{\cref{lem:sig3,lem:sig4}}\\
    &\leq\frac 1 {k^2}\cdot \E_{\lat\sim\msnd}[[\lat\in \rep_\para^{-1}( U)]]+\E_\lat\left[\frac 1 {L^2}\cdot k^{-3+2\epsilon}\right]\\
    &\leq k^{-2}\cdot K\cdot k^{-\delta} + L^{-2}\cdot k^{-3 +2\epsilon}\\
    &\leq \max\{K,L^{-2}\}\cdot k^{-2-\min\{\delta,1-2\epsilon\}}
  \end{align*}
\end{proof}
% \begin{corollary}
%   \label{cor:sigsim}
%   Let $p\neq 0$ be a polynomial. There exists $L,\epsilon>0$ such that
%   $\E_{\mathbf z\sim\msnd}[|\sigma_{k+1}(p(\rep(\para,\lat)))-\sigma_k(p(\rep(\para,\lat)))|^2]< L\cdot k^{-2-\epsilon}$ for all $k\in\nat$ and $\para\in\parasp$.
% \end{corollary}



As a consequence of \cref{lem:sigsim}, Jensen's inequality, a telescoping series argument and the fact that the set of roots of polynomials is negligible \citep{C05} we obtain:
\begin{corollary}
  \label{lem:unifaux}
  Let $0\neq q\from\Real^n\to\Real$ be a polynomial. There exist $L,\epsilon>0$ such that
  $\E_\lat[|\sigma_k(q(\rep_\para(\lat)))-[q(\rep_\para(\lat))>0]|]< L\cdot k^{-\epsilon}$ and $\E_\lat[|\sigma_k(q(\rep_\para(\lat)))-[q(\rep_\para(\lat))\geq 0]|]< L\cdot k^{-\epsilon}$ for all $k$ and $\para\in\parasp$.
\end{corollary}

Note the following elementary fact that for $a_1,\ldots,a_\ell\in(0,1)$ and $b_1,\ldots,b_\ell\in\{0,1\}$,
\begin{align}
  \label{eq:prodsum}
  \left|\prod_{i=1}^\ell a_i-\prod_{i=1}^\ell b_i\right|^2\leq\sum_{i=1}^\ell|a_i-b_i|
\end{align}

\begin{lemma}[Uniform Convergence]
  \label{lem:unifcg}
  Let $0\neq q_1,\ldots,q_\ell:\Real^n\to\Real$ be polynomials and let the absolute value of $h:\Real^m\times\Real^n\to\Real$ be \changed[dw]{bounded by the absolute value of a polynomial}.

  There exist $L,\epsilon>0$ such that
   for all $k\in\nat$ and $\para\in\parasp$,
   \begin{align*}
     \E_\lat\left[\left|h(\para,\lat)\cdot\prod_{i=1}^\ell\sigma_k(q_i(\rep_\para(\lat)))-h(\para,\lat)\cdot\prod_{i=1}^{\ell'}[q_i(\rep_\para(\lat))>0]\cdot\prod_{i=\ell'+1}^{\ell}[q_i(\rep_\para(\lat))\geq 0]\right|\right]< L\cdot k^{-\epsilon}
   \end{align*}
\end{lemma}
\begin{proof}
  By \cref{lem:unifaux,lem:punib} there exist $L,\epsilon>0$ such that ${\bowtie_i}\in\{>,\geq\}$
  \begin{align*}
    \E_\lat[|h(\para,\lat)|^2]&<L\\
    \E_\lat[|\sigma_k(q_i(\rep_\para(\lat)))-[q_i(\rep_\para(\lat))\bowtie_i 0]|]&< L\cdot k^{-\epsilon}&
    \E_\lat[|\sigma_k(q_i(\rep_\para(\lat)))-[q_i(\rep_\para(\lat))\geq 0]|]&< L\cdot k^{-\epsilon}
  \end{align*}
  for all $\para\in\parasp$ and $i\in\{1,\ldots,\ell\}$.
  Therefore,
  \begin{align*}
    &\E_\lat\left[\left|h(\para,\lat)\cdot\prod_{i=1}^\ell\sigma_k(q_i(\rep_\para(\lat)))-h(\para,\lat)\cdot\prod_{i=1}^{\ell}[q_i(\rep_\para(\lat))\bowtie_i 0]\right|\right]\\
    &\leq\sqrt{\E_\lat[|h(\para,\lat)|^2]\cdot\E_\lat\left[\left|\prod_{i=1}^\ell\sigma_k(q_i(\rep_\para(\lat)))-\prod_{i=1}^{\ell}[q_i(\rep_\para(\lat))\bowtie_i 0]\right|^2\right]}&\text{Cauchy-Schwartz}\\
    &\leq\sqrt{L\cdot\sum_{i=1}^{\ell} \E_\lat\left[\left|\sigma_k(q_i(\rep_\para(\lat)))-[q_i(\rep_\para(\lat))\bowtie_i 0]\right|\right]}&\text{\cref{eq:prodsum}}\\
    &\leq\sqrt{L\cdot\ell\cdot L\cdot k^{-\epsilon}}=L\cdot\sqrt\ell\cdot k^{-\frac\epsilon 2}
  \end{align*}
\end{proof}

\subsection{Proof of \cref{prop:unifg}}
\begin{lemma}
  \label{lem:uniaux}
  There exist $L,\epsilon>0$ and integrable $h\from\Real^m\times\Real^n\to\Real$ such that
  $\E_\lat[|\frac{\partial f_k}{\partial \theta_i}(\para,\lat)-h(\para,\lat)|]< L\cdot k^{-\epsilon}$
   for all $k\in\nat$ and $\para\in\parasp$.
%  Let $i\in\{1,\ldots,n\}$. $\E_\lat[\frac{\partial f_k}{\partial \theta_i}(\para,\lat)]$ converges uniformly on $\para\in\parasp$ as $k\to\infty$.
\end{lemma}
\begin{proof}
  First, note that uniform convergence of
  \begin{align*}
    E_\lat\left[\underbrace{\left(\frac{\partial}{\partial\theta_i}p(\para,\lat)\right)}_{\text{polynomial}}\cdot\Psi_k(\rep_\para(\lat))\right]
  \end{align*}
  follows from \cref{lem:unifcg}.
  Besides,
  \begin{align*}
    &E_\lat\left[p(\para,\lat)\cdot\left(\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial\theta_i}(\para,\lat)\right)\right]\\
    &=\sum_{j=1}^n\E_\lat\left[p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\cdot\left(\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\right)\right]&\text{\cref{eq:trick}}\\
    &=\sum_{j=1}^n\int\nd(\lat_{-j})\cdot\int\nd(z_j)\cdot p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\cdot\left(\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\right)\diff z_j\diff \lat_{-j}\\
    &=\sum_{j=1}^n\int\nd(\lat_{-j})\cdot\underbrace{\left[\nd(z_j)\cdot p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\cdot \Psi_k(\rep_\para(\lat))\right]_{-\infty}^\infty}_0\diff\lat_{-j}&\text{integration by parts}\\
    &\quad-\sum_{j=1}^n\int\nd(\lat_{-j})\cdot\int\frac\partial{\partial z_j}\left(\nd(z_j)\cdot p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\cdot\Psi_k(\rep_\para(\lat))\diff z_j\diff\lat_{-j}\\
    &=\sum_{j=1}^n\E_\lat[z_j\cdot p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\cdot\Psi_k(\rep_\para(\lat))]&\frac{\partial\nd}{\partial x}(x)=-x\cdot\nd(x)\\
    &\quad-\sum_{j=1}^n\E_\lat\left[\frac\partial{\partial z_j}\left( p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\cdot\Psi_k(\rep_\para(\lat))\right]
  \end{align*}
  By \cref{lem:velbp} $|\vel_i|$ and $|\frac{\partial\vel_i}{\partial z_j}|$ and are bounded by the absolute value of polynomials and clearly $0\leq\Psi_k(\rep_\para(\lat))\leq 1$. Therefore, uniform convergence of $\E[p(\para,\lat)\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\theta_i}(\para,\lat)]$ follows again from \cref{lem:unifcg}.
\end{proof}

The following is an instance of \citep[Thm.~7.17]{W73}:
\begin{lemma}
  \label{lem:convdiff}
  Suppose $g\from [a,b]\to\Real$ and $g_k\from [a,b]\to\Real$ (for $k\in\nat$) satisfy
  \begin{enumerate}
    \item each $g_k$ is differentiable
    \item $g(x)=\lim_{k\to\infty} g_k(x)$ for all $x\in[a,b]$
    \item $g_k'(x)$ converges uniformly on $[a,b]$.
  \end{enumerate}
  Then $g'(x)=\lim_{k\to\infty}g'_k(x)$ for all $\para\in\parasp$.
\end{lemma}


\begin{corollary}
  \label{cor:convdiff}
  Let $U\subseteq\Real^m$ be compact and $i\in\{1,\ldots,m\}$. Suppose $g\from\Real^m\to\Real$ and $g_k\from\Real^m\to\Real$ (for $k\in\nat$) satisfy
  \begin{enumerate}
    \item each $g_k$ is differentiable
    \item $g(\mathbf x)=\lim_{k\to\infty} g_k(\mathbf x)$ for all $\mathbf x\in U$
    \item $\frac{\partial g_k}{\partial x_i}$ converges uniformly on $U$.
  \end{enumerate}
  Then $\frac{\partial g}{\partial x_i}(\mathbf x)=\lim_{k\to\infty}\frac{\partial g_k}{\partial x_i}(\mathbf x)$ for all $\mathbf x\in U$.
\end{corollary}


\begin{proposition}
  \label{prop:univgaux}
  Let $i\in\{1,\ldots,m\}$.
  There exist $L,\epsilon>0$ such that for all $k\in\nat$ and $\para\in\parasp$,
  \begin{align*}
    \left|\frac{\partial}{\partial \theta_i}\E_\lat[f_k(\para,\lat)]-\frac{\partial}{\partial\theta_i}\E[f(\para,\lat)]\right|< L\cdot k^{-\epsilon}
  \end{align*}
  %
  % \dw{box}
  % $\E_\lat[\frac{\partial f_k}{\partial \theta_j}(\para,\lat)]$ converges uniformly on $\parasp$ to $\frac\partial{\partial\theta_j}\E_\lat[f(\para,\lat)]$.
\end{proposition}
\begin{proof}
  Let $g_k(\para)\defeq\E_{\lat}[f_k(\para,\lat)]$ and $g(\para)\defeq\E_{\lat}[f(\para,\lat)]$.
  By \cref{prop:unb} each $g_k$ is differentiable. By \cref{lem:unifcg}, $g(\para)=\lim_{k\to\infty} g_k(\para)$ for all $\para\in\parasp$.
  By \cref{lem:uniaux}, $\frac{\partial g_k}{\partial\theta_i}$ converges uniformly on $\parasp$ to some $\E_\lat[h(\para,\lat)]$. Therefore,
  by \cref{cor:convdiff},
  \begin{align*}
    \frac\partial{\partial\theta_i}\E_\lat[f(\para,\lat)]=\frac{\partial g}{\partial\theta_i}(\para)=\lim_{k\to\infty}\frac{\partial g_k}{\partial\theta_i}(\para)=\E_\lat[h(\para,\lat)]
  \end{align*}
  for all $\para\in\parasp$.
  Therefore, by \cref{lem:uniaux},
  \begin{align*}
    \left|\frac{\partial}{\partial\theta_i}\E_{\lat}[f_k(\para,\lat)]-\frac\partial{\partial\theta_i}\E[f(\para,\lat)]\right|=
    \left|\E_{\lat}\left[\frac{\partial f_k}{\partial\theta_i}(\para,\lat)\right]-\E[h(\para,\lat)]\right|
    \leq\E_{\lat}\left[\left|\frac{\partial f_k}{\partial\theta_i}(\para,\lat)-h(\para,\lat)\right|\right]
    \leq L\cdot k^{-\epsilon}
  \end{align*}
  for all $\para\in\parasp$.
\end{proof}

\cref{prop:unifg} follows.


\section{Supplementary Materials for \cref{sec:dsgd}}
% \dw{why is old number not re-used?}
% \lo{The problem is solved by invoking the package {\tt thm-restate} before defining the various {\tt newtheorem}.}
% \dw{thanks}

\begin{proof}
  By Taylor's theorem,
  \begin{align*}
    &\E_{\lat_k}[g_{k+1}(\para_{k+1})]\\
    &\leq\E_{\lat_k}[g_k(\para_{k+1})]+k^{-1-\epsilon}\cdot L&\text{\ref{it:univc}}\\
    &\leq\E_{\lat_k}\left[g_k(\para_k)-\gamma_k\cdot\langle\nabla_\para g_k(\para_k),\nabla_\para f_k(\para_k,\lat_k)\rangle+\frac{\gamma_k^2}2\cdot\|\nabla_\para f_k(\para_k,\lat_k)\|^2\cdot\|\Hess g_k\|\right]+k^{-1-\epsilon}\cdot L&\text{Taylor's theorem}\\
    &\leq g_k(\para_k)-\gamma_k\cdot\|\nabla_\para g_k(\para_k)\|^2+\frac{\gamma_k^2}2\cdot L^2+k^{-1-\epsilon}\cdot L&\text{\ref{it:unb}, \ref{it:unibv} and \ref{it:unibH}}\\
    &\leq g_{k}(\para_k)-\gamma_k\cdot\|\nabla_\para g(\para_k)\|^2+\gamma_k\cdot k^{-\epsilon}\cdot L+\frac{\gamma_k^2}2\cdot L^2+k^{-1-\epsilon}\cdot L&\text{\ref{it:univcd}}\\
  \end{align*}
  Hence,
  \begin{align*}
    \gamma_k\|\nabla_\para g(\para_k)\|^2\leq g_{k}(\para_k)-\E_{\lat_k}[g_{k+1}(\para_{k+1})]+r_k
  \end{align*}
  where $r_k\defeq \gamma_k\cdot k^{-\epsilon}\cdot L+\frac{\gamma_k^2}2\cdot L^2+k^{-1-\epsilon}\cdot L$.
  Hence,
  \changed[lo]{
  \begin{align*}
    & \left(\sum_{i=0}^k\gamma_i\right)\cdot
    \min\left( \{ \|\nabla_\para g(\para_0)\|^2 \} \cup \{ \E_{\lat_{i-1}}[\|\nabla_\para g(\para_{i})\|^2] \mid 1 \leq i \leq k\} \right) \\
    & \leq \gamma_0 \, \|\nabla_\para g(\para_0)\|^2 + \sum_{i=1}^k\gamma_{i} \, \E_{\lat_{i-1}}[\|\nabla_\para g(\para_{i})\|^2]\\
    & \leq g_{0}(\para_0)-\E_{\lat_{k}}[g_{k+1}(\para_{k+1})]+\sum_{i=0}^k r_i
  \end{align*}
}
\dw{\begin{align*}
    \left(\sum_{i=0}^k\alpha_i\right)\cdot\min_{i=0}^k \E[\|\nabla_\para g(\para_i)\|^2]\leq\sum_{i=0}^k\alpha_i\E[\|\nabla_\para g(\para_i)\|^2]\leq g_{0}(\para_0)-\E[g_{k+1}(\para_{k+1})]+\sum_{i=0}^k r_i
  \end{align*}
}
\dw{$\alpha$ vs.\ $\gamma$}

where the expectation is taken w.r.t.\ $\lat_0,\ldots,\lat_k\sim\msnd$.
Note that due to $\gamma_k\in\Theta(1/k)$, $\sum_{i\in\nat}\gamma_i=\infty$ and $\sum_{i\in\nat} r_i<\infty$.
Besides, due to $\para_i\in\parasp$, which is bounded, the $g_i(\para_i)$ are bounded from below.
%Therefore, the claim follows immediately.
\changed[lo]{Therefore $\inf \left( \{ \|\nabla_\para g(\para_0)\|^2 \} \cup \{ \E_{\lat_{i-1}}[\|\nabla_\para g(\para_{i})\|^2] \mid i \geq 1\} \right) = 0$.}
\end{proof}



\subsection{Supplementary Materials for \cref{sec:cond}}
\label{app:cond}
Recall the framework set out at the beginning of \cref{app:IUC}.

\begin{proposition}[Uniform Convergence]
  \label{prop:unic}
  There exist $L,\epsilon>0$ such that
  $\E_\lat[|f_{k+1}(\para,\lat)-f_k(\para,\lat)]|]< L\cdot k^{-1-\epsilon}$ for all $k\in\nat$ and $\para\in\parasp$.
\end{proposition}
\begin{proof}
%  Abbreviate $q_i(\para,\lat)\defeq\psi_i(\rep_\para(\lat))$ for $i\in\{1,\ldots,\ell\}$.
  By \cref{lem:sigsim,lem:punib},
  there exist $L,\epsilon>0$ such that for all $\para\in\parasp$ and $i\in\{1,\ldots,\ell\}$,
  \begin{align*}
    \E\left[|p(\para,\lat)|^2\right]&<L&
    \E_\lat\left[\left|\sigma_{k+1}(\psi_i(\rep_\para(\lat)))-\sigma_{k}(\psi_i(\rep_\para(\lat)))\right|^2\right]&< L\cdot k^{-2-\epsilon}
  \end{align*}
  Therefore, using the Cauchy–Schwarz inequality,
  \begin{align*}
    &\E_\lat[|f_{k+1}(\para,\lat)-f_k(\para,\lat)]|]\\
    &\leq\sum_{i=1}^\ell\E_\lat\left[\left|p(\para,\lat)\cdot\left(\prod_{j=i}^\ell\sigma_{k+1}(\psi_j(\rep_\para(\lat)))\right)\cdot\left(\prod_{j=1}^{i-1}\sigma_{k}(\psi_j(\rep_\para(\lat)))\right)-p(\para,\lat)\cdot\left(\prod_{j=i+1}^\ell\sigma_{k+1}(\psi_j(\rep_\para(\lat)))\right)\cdot\left(\prod_{j=1}^{i}\sigma_{k}(\psi_j(\rep_\para(\lat)))\right)\right|\right]\\
    &\leq\sum_{i=1}^\ell\E_\lat\left[\left|p(\para,\lat)\cdot\left(\prod_{j=i+1}^\ell\sigma_{k+1}(\psi_j(\rep_\para(\lat)))\right)\cdot\left(\prod_{j=1}^{i-1}\sigma_{k}(\psi_j(\rep_\para(\lat)))\right)\cdot(\sigma_{k+1}(\psi_i(\rep_\para(\lat)))-\sigma_{k}(\psi_i(\rep_\para(\lat))))\right|\right]\\
%    &\leq\sum_{i=1}^\ell\sqrt{\E_\lat\left[\left|p(\para,\lat)\cdot\left(\prod_{j=i+1}^\ell\sigma_{k+1}(\psi_j(\rep_\para(\lat)))\right)\cdot\left(\prod_{j=1}^{i-1}\sigma_{k}(\psi_j(\rep_\para(\lat)))\right)\right|^2\right]\cdot\E_\lat\left[\left|\sigma_{k+1}(\psi_i(\rep_\para(\lat)))-\sigma_{k}(\psi_i(\rep_\para(\lat)))\right|^2\right]}\\
    &\leq\sum_{i=1}^\ell\sqrt{\E_\lat\left[\left|p(\para,\lat)\right|^2\right]\cdot\E_\lat\left[\left|\sigma_{k+1}(\psi_i(\rep_\para(\lat)))-\sigma_{k}(\psi_i(\rep_\para(\lat)))\right|^2\right]}\\
    &\leq\ell\cdot\sqrt{L\cdot L\cdot k^{-2-\epsilon}}\leq \ell\cdot L\cdot k^{-1-\frac\epsilon 2}
  \end{align*}
\end{proof}

% \subsection{Uniform Bound on Hessian}

% As a consequence of \cref{lem:unifcg} all expectations can be uniformly bounded. Thus, instantiating $h(\para,\lat)\defeq p(\para,\lat)\cdot\vel_i(\para,\lat)$ yields:
\begin{proposition}[Uniform Bound on Hessian]
  \label{prop:unibH}
  Let $i,i'\in\{1,\ldots,m\}$. There exists $L>0$ such that for all $\para\in\parasp$,
  \begin{align*}
    \E_\lat\left[\left|\frac{\partial^2 f_k}{\partial\theta_{i'}\,\partial\theta_i}(\para,\lat)\right|\right]<L
  \end{align*}
\end{proposition}
\begin{proof}
  First, note that
  \begin{align*}
    \E_\lat\left[\left|\frac{\partial^2 p}{\partial\theta_{i'}\,\partial\theta_i}(\para,\lat)\cdot\Psi_k(\rep_\para(\lat))\right|\right]\leq
    \E_\lat\left[\left|\underbrace{\frac{\partial^2 p}{\partial\theta_{i'}\,\partial\theta_i}(\para,\lat)}_{\text{polynomial}}\right|\right]
  \end{align*}
  and the right-hand side can be bounded uniformly by \cref{lem:punib}.
  Besides,
  \begin{align*}
    &\E_\lat\left[\left|\frac{\partial p}{\partial\theta_{i'}}(\para,\lat)\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial\theta_i}(\para,\lat)\right|\right]\\
    &\leq\sum_{j=1}^n\E_\lat\left[\left|\frac{\partial p}{\partial\theta_{i'}}(\para,\lat)\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right|\right]&\text{\cref{eq:trick}}\\
    &\leq\sum_{j=1}^n\E_\lat\left[\left|\left(z_j\cdot\frac{\partial p}{\partial\theta_{i'}}(\para,\lat)\cdot\vel_{i,j}(\para,\lat)+\frac\partial{\partial z_j}\left(\frac{\partial p}{\partial\theta_{i'}}(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\right)\cdot\Psi_k(\rep_\para(\para,\lat))\right|\right]&\text{integration by parts}\\
    &\leq\sum_{j=1}^n\E_\lat\left[\left|z_j\cdot\frac{\partial p}{\partial\theta_{i'}}(\para,\lat)\cdot\vel_{i,j}(\para,\lat)+\frac\partial{\partial z_j}\left(\frac{\partial p}{\partial\theta_{i'}}(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\right|\right]
  \end{align*}
  and the expectations on right-hand side can be bounded uniformly by \cref{lem:velbp,lem:punib}.
  \changed[dw]{(To be completely rigorous, to justify the second step we note that $z_j\mapsto\vel_{i,j}(\para,\lat)$ is a smooth function with a finite number of roots and invoke \cref{lem:intp}.)}

  Finally, applying \cref{eq:trick} in the first and third step,
  \begin{align}
    &\E_\lat\left[\left|p(\para,\lat)\cdot\frac{\partial^2\left(\Psi_k\circ\rep_{(-)}\right)}{\partial\theta_{i'}\,\partial\theta_i}(\para,\lat)\right|\right]\nonumber\\
    &\leq\sum_{j=1}^n\E_\lat\left[\left|p(\para,\lat)\cdot\frac\partial{\partial\theta_{i'}}\left(\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\right|\right]&\nonumber\\
    &\leq\sum_{j=1}^n\E_\lat\left[\left|p(\para,\lat)\cdot\frac{\partial^2\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j\,\partial\theta_{i'}}(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right|\right]+\sum_{j=1}^n\E_\lat\left[\left|p(\para,\lat)\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\frac{\partial\vel_{i,j}}{\partial\theta_{i'}}(\para,\lat)\right|\right]\nonumber\\
    &\leq\sum_{j=1}^n\sum_{j'=1}^n\E_\lat\left[\left|p(\para,\lat)\cdot\frac\partial{\partial z_j}\left(\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_{j'}}(\para,\lat)\cdot\vel_{i',j'}(\para,\lat)\right)\cdot\vel_{i,j}(\para,\lat)\right|\right]&\nonumber\\
    &\quad +\sum_{j=1}^n\E_\lat\left[\left|p(\para,\lat)\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\frac{\partial\vel_{i,j}}{\partial\theta_{i'}}(\para,\lat)\right|\right]
    \label{eq:Hessb}
  \end{align}
  To bound the terms in the first sum uniformly, note that for each $j,j'\in\{1,\ldots,n\}$, using integration by parts twice,
  \begin{align*}
    &\E_\lat\left[\left|p(\para,\lat)\cdot\frac\partial{\partial z_j}\left(\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_{j'}}(\para,\lat)\cdot\vel_{i',j'}(\para,\lat)\right)\cdot\vel_{i,j}(\para,\lat)\right|\right]\\
    &\leq\E_\lat\left[\left|\left(z_j\cdot p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)+\frac\partial{\partial z_j}\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\right)\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_{j'}}(\para,\lat)\cdot\vel_{i',j'}(\para,\lat)\right|\right]\\
    &\leq\E_\lat\left[\left|z_{j'}\cdot\left(z_j\cdot p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)+\frac\partial{\partial z_j}\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\right)\cdot\Psi_k(\rep_\para(\lat))\cdot\vel_{i',j'}(\para,\lat)\right|\right]\\
    &\quad+\E_\lat\left[\left|\frac\partial{\partial z_{j'}}\left(\left(z_j\cdot p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)+\frac\partial{\partial z_j}\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\right)\cdot\vel_{i',j'}(\para,\lat)\right)\cdot\Psi_k(\rep_\para(\lat))\right|\right]\\
    &\leq\E_\lat\left[\left|z_{j'}\cdot\left(z_j\cdot p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)+\frac\partial{\partial z_j}\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\right)\cdot\vel_{i',j'}(\para,\lat)\right|\right]\\
    &\quad+\E_\lat\left[\left|\frac\partial{\partial z_{j'}}\left(\left(z_j\cdot p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)+\frac\partial{\partial z_j}\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)\right)\cdot\vel_{i',j'}(\para,\lat)\right)\right|\right]
  \end{align*}
  and the expectations can be bounded uniformly by \cref{lem:velbp,lem:punib}.

  The other expectations in \cref{eq:Hessb} can be bounded similarly.
\end{proof}

\begin{proposition}[Uniform Bound on ``Variance'']
  \label{prop:unibv}
  Let $i\in\{1,\ldots,m\}$. There exists $L>0$ such that for all $\para\in\parasp$,
  \begin{align*}
    \E_\lat\left[\left|\frac{\partial f_k}{\partial\theta_i}(\para,\lat)\right|^2\right]<L
  \end{align*}
\end{proposition}
\begin{proof}
  \begin{align*}
    &\E_\lat\left[\left|p(\para,\lat)\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial\theta_i}(\para,\lat)\right|^2\right]\\
    &\leq n\cdot\sum_{j=1}^n\E_\lat\left[\left|p(\para,\lat)\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right|^2\right]&\text{\cref{eq:trick}}\\
    &\leq n\cdot\sum_{j=1}^n\E_\lat\left[\left|z_j\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2\cdot\Psi_k(\rep_\para(\lat))\right|\right]\\
    &\quad+ n\cdot\sum_{j=1}^n\E_\lat\left[\left|\frac\partial{\partial z_j}\left(\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2\right)\cdot\Psi_k(\rep_\para(\lat))\right|\right]&\text{integration by parts}\\
    &\leq n\cdot\sum_{j=1}^n\E_\lat\left[\left|z_j\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2\right|\right]\\
    &\quad+ n\cdot\sum_{j=1}^n\E_\lat\left[\left|\frac\partial{\partial z_j}\left(\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2\right)\right|\right]\\
    &\leq n\cdot\sum_{j=1}^n\E_\lat\left[\left|\left(z_j^2\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2+\frac{\partial}{\partial z_j}\left(z_j\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2\right)\right)\cdot \Psi_k(\rep_\para(\lat))\right|\right]\\
    &\quad+ n\cdot\sum_{j=1}^n\E_\lat\left[\left|z_j\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2\right|\right]&\text{integration by parts}\\
    &\leq n\cdot\sum_{j=1}^n\E_\lat\left[\left|z_j^2\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2\right|\right]+ n\cdot\sum_{j=1}^n\E_\lat\left[\left|\frac{\partial}{\partial z_j}\left(z_j\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2\right)\right|\right]\\
    &\quad+ n\cdot\sum_{j=1}^n\E_\lat\left[\left|z_j\cdot\frac{\partial\left(\Psi_k\circ\rep_{(-)}\right)}{\partial z_j}(\para,\lat)\cdot\left(p(\para,\lat)\cdot\vel_{i,j}(\para,\lat)\right)^2\right|\right]\\
  \end{align*}
  The terms in the third sum can be bounded uniformly as before by once again using integration by parts. For the others it follows directly from \cref{lem:velbp,lem:punib}.
\end{proof}




\section{Properties of Polynomials}
\begin{assumption}
  Throughout this section we assume that $\parasp\subseteq\Real^m$ is compact.
\end{assumption}
\subsection{Uniform Bounds}

\begin{lemma}
  \label{lem:puniq}
  For $\para\in\parasp$, let $p_\para\from\Real^n\to\Real$ be a polynomial the coefficients of which depend continuously on $\para$.

  Then there exists a polynomial $q\from\Real^n\to\Real$ such that $|p_\para|\leq |q|$ for all $\para\in\parasp$.
\end{lemma}
\begin{proof}
  First, suppose $f\from\parasp\to\Real$, the coefficient function of a monomial, is continuous and let $k_1,\ldots,k_n\in\nat$.
  Since, $|f|$ is continuous and $\parasp$ is compact there exists $M\defeq\max_{\para\in\parasp}|f(\para)|$.
  Then
  \begin{align*}
    \left|f(\para)\cdot\prod_{i=1}^n z_i^{k_i}\right|\leq M\cdot |z_i^{k_i}|
  \end{align*}

  The claim follows by linearity.
\end{proof}


\begin{lemma}
  \label{lem:punib}
  For $\para\in\parasp$, let $p_\para\from\Real^n\to\Real$ be a polynomial the coefficients of which depend continuously on $\para$.

  Then there exists $M>0$ such that for all $\para\in\parasp$, $\E_{\lat\sim\msnd}[|p_\para(\lat)|]<M$.
\end{lemma}
\begin{proof}
  By \cref{lem:puniq} there exists a polynomial $q\from\Real^n\to\Real$ such that for all $\para\in\parasp$, $|p_\para|\leq|q|$. Furthermore, (absolute) moments of normals are finite. Therefore $|q|$ is integrable and $M\defeq\E_{\lat\sim\msnd}[|q(\lat)|]$ is well-defined.
  %
  %
  % First, suppose $f\from\parasp\to\Real$ is continuous and let $k_1,\ldots,k_n\in\nat$. Then
  % \begin{align*}
  %   \parasp\mapsto\E_{\lat\sim\msnd}\left[\left|f(\para)\cdot\prod_{i=1}^n z_i^{k_i}\right|\right]=|f(\para)|\cdot\underbrace{\prod_{i=1}^n\E_{z_i\sim\nd(0,1)}\left[\left|z_i^{k_i}\right|\right]}_{\text{constant}}
  % \end{align*}
  % is well-defined because the moments of the standard normal are finite and continuous. Therefore, the function is bounded because $\parasp\subseteq\Real^m$ is compact.
  %
  % The claim follows by linearity.
\end{proof}

\subsection{Behaviour Near Roots}

\iffalse
\begin{lemma}
  \label{lem:roots1}
  Let $\epsilon>0$ and $p_\para(z)=\sum_{i=0}^n a_{\para,i}\cdot z^i$ be a (univariate) polynomial such that each $\para\mapsto a_{\para,i}$ is continuous and $a_{\para,n}\neq 0$ for all $\para\in\parasp$.

   Then $L\defeq\min |a_{\para,n}|>0$ and for all $\para\in\parasp$ and $k\in\nat$ there exist $U\subseteq\Real$ such that $\Leb(U)\leq 2n\cdot k^{-\frac\epsilon n}$ and for all $z\in\Real\setminus U$, $|p_\para(z)|>L\cdot k^{-\epsilon}$.
\end{lemma}
\begin{proof}
  $L>0$ follows from compactness of $\parasp$ and continuity of $\para\mapsto a_{\para,n}$.

  By the fundamental theorem of algebra $p_\para$ has the form $p_\para(z)= a_{\para,n}\cdot\prod_{i=1}^n (z-b_{\para,i})$, where each $b_{\para,i}\in\mathbb C$.

  Now, suppose $\para\in\parasp$ and $k\in\nat$. Define
  $U\defeq\bigcup_{i=1}^n\{z\in\Real\mid|z-b_{\para,i}|\leq k^{-\frac\epsilon n}\}$. Clearly, $\Leb(U)\leq 2 n\cdot k^{-\frac\epsilon n}$. Furthermore, for $z\in\Real\setminus U$,
  \begin{align*}
    |p_\para(z)|&=|a_{\para,n}|\cdot\prod_{i=1}^n |z-b_{\para,i}|
    >L\cdot \prod_{i=1}^n k^{-\frac\epsilon n}
    = L\cdot k^{-\epsilon}\qedhere
  \end{align*}
\end{proof}
\dw{$L$ vs. $a_n$}

The proof of the following has a similar flavour to the proof of the fact that the roots of non-trivial polynomials have measure $0$ \cite{C05}:
\begin{lemma}
  \label{lem:polyr}
  Let $\mu$ be the standard Gaussian probability measure on $\Real^n$, i.e.\ the measure with pdf $\msnd$.\\
  Let $0\neq p_\para\from\Real^n\to\Real$ be a polynomial for $\para\in\parasp$ the coefficients of which depend continuously on $\para$, and let $\epsilon>0$.\\
  There exist $K,L,\delta>0$ such that
  for all $k\in\nat$ and $\para\in\parasp$ there exist $U\subseteq\Real^n$ such that $\mu(U)\leq K\cdot k^{-\delta}$ and for all $\lat\in\Real^n\setminus U$, $|p_\para(\lat)|>L\cdot k^{-\epsilon}$.
\end{lemma}
\begin{proof}
  We prove the claim by induction on $n$. For $n=0$ this is trivial. Hence, suppose $n\geq 0$, $\epsilon>0$ and
  \begin{align*}
    p_\para(z_1,\ldots,z_{n+1})=\sum_{i=0}^\ell p_{\para,i}(z_1,\ldots,z_n)\cdot z_{n+1}^i
    =p_{\para,(z_1,\ldots,z_n)}(z_{n+1})
  \end{align*}
  where each $p_{\para,i}\from\Real^n\to\Real$ is a polynomial the coefficients of which depend continuously on $\para$.

  There exist compact $\parasp_i\subseteq\Real^m$ such that \dw{to be completely rigorous this also needs to depend continuously/measurably on the $z_i$}
  \begin{enumerate}
    \item $\bigcup_{i=0}^\ell\parasp_i=\parasp$,
    \item for each $\para\in\parasp_i$, $p_{\para,i}\neq 0$
    \item $\para\in\parasp_i$ and $j>i$ implies $p_{\para,i}=0$.
  \end{enumerate}
  \dw{details}

  Let $K_i,L_i,\delta_i>0$ be the constants the inductive hypothesis yields for $p_{\para,i}$, $\parasp_i$ and $\frac\epsilon 2$.
  Define
  \begin{align*}
    K&\defeq \max_{i=0}^\ell K_i+2\ell& L&\defeq\min_{i=0}^\ell L_i&\delta&\defeq\min_{i=0}^\ell\left\{\delta_i,\frac\epsilon{2\ell}\right\}
  \end{align*}

  Suppose $k\in\nat$ and $\para\in\parasp_i$.

  The inductive hypothesis for $p_{\para,i}$, $\frac\epsilon 2$, $k\in\nat$ and $\para\in\parasp_i$ yields $U_i\subseteq\Real^n$ such that $\mu(U_i)\leq K_i\cdot k^{-\delta_i}$ and for all $(z_1,\ldots,z_n)\in\Real^n\setminus U_i$, $|p_{\para,i}(z_1,\ldots,z_n)|>L_i\cdot k^{-\frac\epsilon 2}$.


  Besides, for each $(z_1,\ldots,z_n)\in\Real^n\setminus U_i$, applying \cref{lem:roots1} to $p_{\para,(z_1,\ldots,z_n)}$ and $\frac\epsilon 2$ and $\parasp_i$ there exists $U_{(z_1,\ldots,z_n)}\subseteq\Real$ such that
  \begin{align}
    \Leb\left(U_{(z_1,\ldots,z_n)}\right)&\leq 2 i\cdot k^{-\frac\epsilon{2 i}}\leq 2\ell\cdot k^{-\frac\epsilon{2\ell}}\\
    p_{\para,(z_1,\ldots,z_n)}(z_{n+1})&>
    % |p_{\para,i}(z_1,\ldots,z_n)|\cdot k^{-\frac\epsilon 2}>
    L_i\cdot k^{-\epsilon}
  \end{align}
  for all $z_{n+1}\in\Real\setminus U_{(z_1,\ldots,z_n)}$.


  Define
  \begin{align*}
    U\defeq\left\{(z_1,\ldots,z_{n+1})\in\Real^{n+1}\mid (z_1,\ldots,z_n)\in U_i \text{ or }z_{n+1}\in U_{(z_1,\ldots,z_n)}\right\}
  \end{align*}
  Note
  \begin{align*}
    \mu(U)&\leq\mu(U_i\times\Real)+\mu(\{(z_1,\ldots,z_{n+1})\in\Real^{n+1}\mid z_{n+1}\in U_{(z_1,\ldots,z_n)}\})\\
    &\leq K_i\cdot k^{-\delta_i}+2\cdot \ell\cdot k^{-\frac\epsilon{2\ell}}\\
    &\leq K\cdot k^{-\delta}
  \end{align*}
  \changed[dw]{because $\mu$ is a probability measure and the standard normal gaussian density is bounded by $1$.}

  Besides, if $(z_1,\ldots,z_{n+1})\in\Real^{n+1}\setminus U$ and $\para\in\parasp_i$ then $(z_1,\ldots,z_n)\in\Real^n\setminus U_i$ and $z_{n+1}\in\Real\setminus U_{(z_1,\ldots,z_n)}$. Therefore,
  \begin{align*}
    |p_\para(z_1,\ldots,z_{n+1})|&=|p_{\para,(z_1,\ldots,z_n)}(z_{n+1})|> L_i\cdot k^{-\epsilon}\geq L\cdot k^{-\epsilon} \qedhere
  \end{align*}
\end{proof}
\fi


\begin{lemma}
  \label{lem:roots1}
  Let $\epsilon>0$ and $p(z)=\sum_{i=0}^n a_{i}\cdot z^i$ be a (univariate) polynomial such that $a_{n}\neq 0$.

   Then for all $k\in\nat$ there exist $U\subseteq\Real$ such that $\Leb(U)\leq 2n\cdot k^{-\frac\epsilon n}$ and for all $z\in\Real\setminus U$, $|p(z)|>a_n\cdot k^{-\epsilon}$.
\end{lemma}
\begin{proof}
  By the fundamental theorem of algebra $p$ has the form $p(z)= a_{n}\cdot\prod_{i=1}^n (z-b_{i})$, where each $b_{i}\in\mathbb C$.

  Now, suppose $k\in\nat$. Define
  $U\defeq\bigcup_{i=1}^n\{z\in\Real\mid|z-b_{i}|\leq k^{-\frac\epsilon n}\}$. Clearly, $\Leb(U)\leq 2 n\cdot k^{-\frac\epsilon n}$. Furthermore, for $z\in\Real\setminus U$,
  \begin{align*}
    |p(z)|&=|a_{n}|\cdot\prod_{i=1}^n |z-b_{i}|
    >L\cdot \prod_{i=1}^n k^{-\frac\epsilon n}
    = L\cdot k^{-\epsilon}\qedhere
  \end{align*}
\end{proof}
%
% \begin{assumption}
%   \label{ass:probm}
%   Suppose $M>0$, $\parasp\subseteq\Real^m$ and $f^{(n)}_\para\from\Real^n\to\Real_{+}$ for $n\in\nat$ are such that for all $n\in\nat$ and $\para\in\parasp$, $x_1,\ldots,x_n\in\Real$,
%   \begin{enumerate}
%     \item $f^{(n)}_\para(x_1,\ldots,x_n)\leq M$
%     \item $\int f^{(n+1)}_\para(x_1,\ldots,x_{n+1})\diff x_{n+1}=1$
%   \end{enumerate}
% \end{assumption}
% Thus, each $(x_1,\ldots,x_n)\mapsto\prod_{i=1}^n f_i(x_1,\ldots,x_i)$ is the density of a probability measure $\nu_\para^{(n)}$. Besides,
% \begin{enumerate}
%   \item for measurable $U\subseteq\Real^n$, $\nu_{n+1}(U\times\Real)=\nu_n(U)$
%   \item if for each $x_1,\ldots,x_n\in\Real$ $U_{(x_1,\ldots,x_n)}\subseteq\Real$ is such that $\Leb(U_{(x_1,\ldots,x_n)})\leq N$ then $\nu_{n+1}(\{(x_1,\ldots,x_{n+1})\mid x_{n+1}\in U_{(x_1,\ldots,x_n)}\})\leq M\cdot N$.
% \end{enumerate}
%
% \begin{assumption}
%   Let $M>0$ and for $j\in\{1,\ldots,n\}$ let
%   $\phi^{(j)}_{\para}\from\Real^j\to\Real^n$ be a diffeomorphic polynomial such that
%   \begin{enumerate}
%     \item for all $\para\in\parasp$ and $z_1,\ldots,z_j\in\Real$, $\left|\frac{\partial\phi^{(j)}}{\partial z_j}(\para,(z_1,\ldots,z_j))\right|\geq M$
% %    \item for all $j'>j$, $\para\in\parasp$ and $\lat\in\Real^n$, $\left|\frac{\partial\phi^{(j)}}{\partial z_{j'}}(\para,\lat)\right|=0$
%   \end{enumerate}
% \end{assumption}
%
% For $j\in\{1,\ldots,n\}$, let $\nu^{(j)}$ to be the probability measure on $\Real^j$ with density
% $(z_1,\ldots,z_j)\mapsto\prod_{i=1}^j \nd({\phi^{(i)}_\para}^{-1}(z_1,\ldots,z_i))\cdot\frac{\partial\phi^{(i)}}{\partial z_i}(\para,(z_1,\ldots,z_i))$.
% Note that
% \begin{enumerate}
%   \item for measurable $U\subseteq\Real^n$, $\nu_{n+1}(U\times\Real)=\nu_n(U)$
%   \item if for each $x_1,\ldots,x_n\in\Real$ $U_{(x_1,\ldots,x_n)}\subseteq\Real$ is such that $\Leb(U_{(x_1,\ldots,x_n)})\leq N$ then $\nu_{n+1}(\{(x_1,\ldots,x_{n+1})\mid x_{n+1}\in U_{(x_1,\ldots,x_n)}\})\leq M\cdot N$.
% \end{enumerate}


\dw{replace $x$, $\alpha$}

\dw{CHECK}
\begin{lemma}
  \label{lem:polyr}
  Let $M>0$ and for $j\in\{1,\ldots,n\}$ and $\para\in\parasp$, let $\nu_\para^{(j)}$ be a probability measure on $\Real^j$ satisfying
  \begin{enumerate}
    \item for measurable $U\subseteq\Real^{j}$, $\nu_\para^{(j+1)}(U\times\Real)=\nu_\para^{(j)}(U)$
    \item if for each $x_1,\ldots,x_j\in\Real$ and $U_{(x_1,\ldots,x_j)}\subseteq\Real$ is such that $\Leb(U_{(x_1,\ldots,x_j)})\leq N$ then $\nu_\para^{(j+1)}(\{(x_1,\ldots,x_{j+1})\mid x_{j+1}\in U_{(x_1,\ldots,x_j)}\})\leq M\cdot N$.
  \end{enumerate}

  Furthermore, let
  $0\neq p\from\Real^n\to\Real$ be a polynomial and $\epsilon>0$.

  Then there exists $K,L,\delta>0$ such that
  for all $k\in\nat$ and $\para\in\parasp$ there exist $U\subseteq\Real^n$ such that $\nu_\para^{(n)}(U)\leq K\cdot k^{-\delta}$ and for all $\mathbf x\in\Real^n\setminus U$, $|p(\mathbf x)|>L\cdot k^{-\epsilon}$.
\end{lemma}
\begin{proof}
  We prove the claim by induction on $n$. For $n=0$ this is trivial. Hence, suppose $n\geq 0$, $\epsilon>0$ and
  \begin{align*}
    p(x_1,\ldots,x_{n+1})=\sum_{i=0}^\ell p_i(x_1,\ldots,x_n)\cdot x_{n+1}^i
    =p_{(x_1,\ldots,x_n)}(x_{n+1})
  \end{align*}
  where each $p_i\from\Real^n\to\Real$ is a polynomial and $p_\ell\neq 0$.



  Let $K_\ell,L_\ell,\delta_\ell>0$ be the constants the inductive hypothesis yields for $p_\ell$.
  Define
  \begin{align*}
    K&\defeq M\cdot K_\ell+2 \ell\cdot M& L_\ell&\defeq L&\delta&\defeq\min\left\{\delta_\ell,\frac\epsilon{2\ell}\right\}
  \end{align*}

  Suppose $k\in\nat$ and $\para\in\parasp$.
  For each $(x_1,\ldots,x_n)\in\Real^n$, applying \cref{lem:roots1} to $p_{(x_1,\ldots,x_n)}$ and $\frac\epsilon 2$ there exists $U_{(x_1,\ldots,x_n)}\subseteq\Real$ such that
  \begin{align}
    \Leb\left(U_{(x_1,\ldots,x_n)}\right)&\leq 2\ell\cdot k^{-\frac\epsilon{2\ell}}\\
    p_{(x_1,\ldots,x_n)}(x_{n+1})&> |p_\ell(x_1,\ldots,x_n)|\cdot k^{-\frac\epsilon 2}
  \end{align}
  for all $x_{n+1}\in\Real\setminus U_{(x_1,\ldots,x_n)}$.

  The inductive hypothesis for $p_\ell$ and $\frac\epsilon 2$ yields $U_\ell\subseteq\Real^n$ such that $\nu_\para^{(n)}(U_\ell)\leq K_\ell\cdot k^{-\delta}$ and for all $(x_1,\ldots,x_n)\in\Real^n\setminus U$, $|p_\ell(x_1,\ldots,x_n)|>L_\ell\cdot k^{-\frac\epsilon 2}$.

  Define
  \begin{align*}
    U\defeq\left\{(x_1,\ldots,x_{n+1})\in\Real^{n+1}\mid (x_1,\ldots,x_n)\in U_\ell\text{ or }x_{n+1}\in U_{(x_1,\ldots,x_n)}\right\}
  \end{align*}
  Note
  \begin{align*}
    \nu_\para^{(n+1)}(U)&\leq\nu_\para^{(n+1)}(U_\ell\times\Real)+\nu_\para^{(n+1)}(\{(x_1,\ldots,x_{n+1})\in\Real^{n+1}\mid x_{n+1}\in U_{(x_1,\ldots,x_n)}\})\\
    &\leq M\cdot K_\ell\cdot k^{-\delta_\ell}+2 M\cdot \ell\cdot k^{-\frac\epsilon{2\ell}}\\
    &\leq K\cdot k^{-\delta}
  \end{align*}

  Besides, if $(x,\ldots,x_{n+1})\in\Real^{n+1}\setminus U$ then $(x_1,\ldots,x_n)\in\Real^n\setminus U_\ell$ and $x_{n+1}\in\Real\setminus U_{(x_1,\ldots,x_n)}$. Therefore,
  \begin{align*}
    |p(x_1,\ldots,x_{n+1})|&=|p_{(x_1,\ldots,x_n)}(x_{n+1})|> |p_\ell(x_1,\ldots,x_n)|\cdot k^{-\frac\epsilon 2}> L_\ell\cdot k^{\epsilon}=L\cdot k^{-\epsilon} \qedhere
  \end{align*}
\end{proof}


\begin{corollary}
  \label{cor:polyr}
%  Let $\nu_n$ be a probability measure on $\Real^n$.
Let $\phi_\para^{(1)},\ldots,\phi_\para^{(n)}$ be as in \cref{ass:diff} of \cref{ass:ass}, let $0\neq p\from\Real^n\to\Real$ be a polynomial and $\epsilon>0$.

Then there exists $K,L,\delta>0$ such that
  for all $k\in\nat$ and $\para\in\parasp$ there exist $U\subseteq\Real^n$ such that $\E_{\lat\sim\msnd}[[\lat\in\rep_\para^{-1}(U)]]\leq K\cdot k^{-\delta}$ and for all $\mathbf x\in\Real^n\setminus U$, $|p(\mathbf x)|>L\cdot k^{-\epsilon}$.
\end{corollary}
\begin{proof}
  For $j\in\{1,\ldots,n\}$, let $\nu^{(j)}$ to be the probability measure on $\Real^j$ with density
  \begin{align*}
    (z_1,\ldots,z_j)\mapsto\prod_{i=1}^j \nd\left(\left({\phi^{(i)}_\para}\right)^{-1}(z_1,\ldots,z_i)\right)\cdot\frac{\partial\phi^{(i)}}{\partial z_i}(\para,(z_1,\ldots,z_i))
  \end{align*}
  Note that $\E_{\lat\sim\msnd}[[\lat\in\rep_\para^{-1}(U)]]=\nu_\para(U)$ and by \cref{lem:lbdet} the conditions of \cref{lem:polyr} are satisfied.
\end{proof}



\iffalse
\subsection{Large Values}

% \begin{lemma}
%   Let $\parasp\subseteq\Real^m$ be compact and $p\from\Real^m\times\Real\to\Real$ be a polynomial.
%
%   There exists $L,M,\epsilon,\eta>0$ such that
%   for every $k\in\nat$ there exists $U\subseteq\Real$ such that $\E_{\lat}[[\lat\in U]]< L\cdot k^{-\delta}$ and for $\lat\in\Real\setminus U$, $|p(\para,\lat)|< M\cdot k^\eta$.
% \end{lemma}
% \begin{proof}
%   Suppose $p(\lat,z)=\sum_{i=0}^n a_{\para,i}\cdot x^i$.
%   Note that $\{\mu_\para\mid\para\in\parasp\}\subseteq [b,c]$ is compact and $\inf_{\para\in\parasp}\sigma_\para>0$.
%   Besides, $\infty>\sup_{i\in\{1,\ldots,n\}}\sup_{\para\in\parasp}|a_{\para,i}|=: a$.
%
%   Suppose $k\in\nat$.
%   Let $V\defeq [b-k^\delta,c+k^\delta]$
%   $U\defeq\Real\setminus U$.
%   Note that $x\in V$, $|x|\leq 2\cdot\max\{1,|b|,|c|,k^\delta\}$.
%   Thus,
%   if $\lat\in\Real\setminus U$, $\lat\in V$ and
%   \begin{align*}
%     |p(\para,z)|\leq\sum_{i=1}^n |a_{\para,i}\cdot x^i|\leq \sum_{i=1}^n a\cdot |x_i|^i\leq n\cdot a\cdot 2\cdot\max\{1,|b|,|c|,k^\delta\}^n
%   \end{align*}
%   So, we can set $\eta\defeq n\cdot\delta$.
%
%   \begin{align*}
%     \int_{-\infty}^{b-k^\delta} \nd(x\mid\mu_\para,\sigma_\para)\diff x&\leq \frac {\sigma_\para^2}{k^\delta}\cdot\int_U -\frac {2(x-\mu_\para)}{2\sigma_\para^2}\cdot\nd(x\mid\mu_\para,\sigma_\para)\\
%     &\leq \frac {\sigma_\para^2}{k^\delta}\cdot\left[\nd(x\mid\mu_\para,\sigma_\para)\right]_{-\infty}^{b-k^\delta}\\
%     &\leq \frac {\sigma_\para^2}{k^\delta}
%   \end{align*}
%   Similarly, $\int_{c-k^\delta}^\infty \nd(x\mid\mu_\para,\sigma_\para)\diff x\leq \frac {\sigma_\para^2}{k^\delta}$.
% \end{proof}


\begin{lemma}
  \label{lem:polylarge}
  Let $p\from\Real^m\times\Real^n\to\Real$ be a polynomial and $\eta>0$.

  There exist $L,M,\delta>0$ such that
  for every $k\in\nat$ there exists $U\subseteq\Real^n$ such that $\E_{\lat}[[\lat\in U]]< L\cdot k^{-\delta}$ and for $\lat\in\Real^n\setminus U$, $|p(\para,\lat)|< M\cdot k^\eta$.
\end{lemma}
\begin{proof}
  Suppose $p(\para,\lat)=\sum_{i=1}^\ell a_{\para,i}\cdot x_1^{j_{i,0}}\cdots x_m^{j_{i,m}}$.
  Let $j\defeq\max_{i=1}^\ell j_{i,0}+\cdots+ j_{i,m}$ be its degree.

  Note that $\{\mathbf\mu_\para\mid\para\in\parasp\}\subseteq [b,c]^n$ is compact and $\sigma\defeq\min_{i=1}^m\inf_{\para\in\parasp}\sigma_\para>0$.
  Besides, $\infty>\sup_{i\in\{1,\ldots,n\}}\sup_{\para\in\parasp}|a_{\para,i}|=: a$.
  Let $\delta\defeq \frac\eta j$.

  Suppose $k\in\nat$.
  Let $V\defeq [b-k^\delta,c+k^\delta]^n$,
  $U\defeq\Real\setminus V$.
  Note that $\lat\in V$, $|z_i|\leq 2\cdot\max\{1,|b|,|c|,k^\delta\}$.
  Thus,
  if $\lat\in\Real\setminus U$, $\lat\in V$ and for $\para\in\parasp$,
  \begin{align*}
    |p(\para,\lat)|\leq\sum_{i=1}^\ell\left |a_{\para,i}\cdot z_0^{j_{i,0}}\cdots z_m^{j_{i,m}}\right|\leq \sum_{i=1}^\ell a\cdot |z_0|^{j_{i,0}}\cdots |z_m|^{j_{i,m}}\leq\ell\cdot a\cdot 2\cdot\max\{1,|b|,|c|,k^\delta\}^{j}
  \end{align*}

  Let $U_i\defeq \Real\times\cdots\times\Real\times (-\infty,b-k^\delta)\times\Real\times \cdots\times\Real$ and $U_i'\defeq \Real\times\cdots\times\Real\times (c+k^\delta,\infty)\times\Real\times \cdots\times\Real$. Note that $U=U_1\cup\cdots\cup U_n\cup U'_1\cup\cdots\cup U'_n$. Besides,
  \begin{align*}
    &\E_{\lat}[[\lat\in U_i]]
    &=\int_{-\infty}^\infty\nd(z_1\mid\mu_\para^{(1)},\sigma_\para^{(1)})\cdot\int_{-\infty}^\infty\cdots\int_{-\infty}^{b-k^\delta}\nd(z_i\mid\mu_\para^{(i)}(z_1,\ldots,z_{i-1}),\sigma_\para^{(i)})\cdot\int_{-\infty}^\infty\cdots\int_{-\infty}^\infty \nd(z_n\mid\mu_\para^{(n)}(z_1,\ldots,z_{n-1}),\sigma_\para^{(n)})\diff\lat\\
    &=\int_{-\infty}^\infty\nd\left(z_1\mid\mu_\para^{(1)},\sigma_\para^{(1)}\right)\cdot\int_{-\infty}^\infty\cdots\int_{-\infty}^{b-k^\delta}\nd\left(z_i\mid\mu_\para^{(i)}(z_1,\ldots,z_{i-1}),\sigma_\para^{(i)}\right)\cdot 1\diff z_i\cdots\diff z_1\\
    &\leq\int_{-\infty}^\infty\nd\left(z_1\mid\mu_\para^{(1)},\sigma_\para^{(1)}\right)\cdot\int_{-\infty}^\infty\cdots\frac{\left(\sigma_\para^{(i)}\right)^2}{k^\delta}\int_{-\infty}^{b-k^\delta}-\frac {2\cdot\left(x-\mu_\para^{(i)}(z_1,\ldots,z_{i-1})\right)}{2\left(\sigma^{(i)}_\para\right)^2}\cdot\nd\left(z_i\mid\mu_\para^{(i)}(z_1,\ldots,z_{i-1}),\sigma_\para^{(i)}\right)\diff z_i\cdots\diff z_1\\
    &=\int_{-\infty}^\infty\nd\left(z_1\mid\mu_\para^{(1)},\sigma_\para^{(1)}\right)\cdot\int_{-\infty}^\infty\cdots\frac{\left(\sigma_\para^{(i)}\right)^2}{k^\delta}\left[\nd\left(z_i\mid\mu_\para^{(i)}(z_1,\ldots,z_{i-1}),\sigma_\para^{(i)}\right)\right]_{-\infty}^{b-k^\delta}\diff z_i\cdots\diff z_1\\
    &\leq\int_{-\infty}^\infty\nd\left(z_1\mid\mu_\para^{(1)},\sigma_\para^{(1)}\right)\cdot\int_{-\infty}^\infty\cdots\frac{\left(\sigma_\para^{(i)}\right)^2}{k^\delta}\diff z_i\cdots\diff z_1\\
    &=\frac{\left(\sigma_\para^{(i)}\right)^2}{k^\delta}\leq\frac{\sigma^2}{k^\delta}
  \end{align*}
  Similarly, $\E_\lat[[\lat\in U_i']]\leq \frac{\sigma^2}{k^\delta}$. Therefore
  $\E_\lat[[\lat\in U]]\leq 2n\cdot\frac{\sigma^2}{k^\delta}$.
\end{proof}
\fi

\section{Properties of Sigmoid}
\dw{Question: can we use other smoothings}

Note that for $k\in\nat$,
\begin{align}
  \label{eq:sqrt}
  \sqrt{k+1}-\sqrt k\leq\frac 1{\sqrt k}
\end{align}
Besides, for $x\in\Real$ and $y\in\Real_+$,
\begin{align}
  \sigma'(x)=\sigma(x)\cdot(1-\sigma(x))&\leq1-\sigma(x)\label{eq:sig2}\\
  1-\sigma(y)&\leq\frac 1 y\label{eq:sig1}\\
  1-\sigma(y)&\leq\frac 1 {y^2}\label{eq:sigs1}
\end{align}

\begin{lemma}
  \label{lem:sig3}
  Let $k\in\nat$ and $y\in\Real$, then $|\sigma_{k+1}(y)-\sigma_k(y)|\leq\frac 1 k$.
\end{lemma}
\begin{proof}
  Note that
  $|\sigma_{k+1}(-y)-\sigma_k(-y)|=|1-\sigma_{k+1}(y)-(1-\sigma_k(y))|$. Therefore, it suffices to consider $y>0$.
  By Taylor's theorem there exists $\zeta\in (\sqrt k\cdot y,\sqrt{k+1}\cdot y)$ such that
  \begin{align*}
    |\sigma_{k+1}(y)-\sigma_k(y)|&=\sigma'(\zeta)\cdot(\sqrt{k+1}-\sqrt k)\cdot y\\
    &\leq \sigma'(\sqrt k\cdot y)\cdot(\sqrt{k+1}-\sqrt k)\cdot y&\sigma'_{|\Real_+}\text{ decreasing}\\
    &\leq (1-\sigma(\sqrt k\cdot y))\cdot(\sqrt{k+1}-\sqrt k)\cdot y&\text{\cref{eq:sig2}}\\
    &\leq \frac 1{\sqrt k\cdot y}\cdot(\sqrt{k+1}-\sqrt k)\cdot y&\text{\cref{eq:sig1}}\\
    &\leq \frac 1{\sqrt k\cdot y}\cdot\frac 1{\sqrt k}\cdot y&\text{\cref{eq:sqrt}}\\
    &=\frac 1 k
  \end{align*}
\end{proof}

\begin{lemma}
  \label{lem:sig4}
  Let $L,\epsilon>0$, $k\in\nat$ and $y\in\Real$ be such that $|y|>L\cdot k^{-\epsilon}$, then $|\sigma_{k+1}(y)-\sigma_k(y)|\leq\frac 1 L\cdot k^{-\frac 3 2+\epsilon}$.
\end{lemma}
\begin{proof}
  Again, it suffices to consider $y>0$.
  % First, suppose $L\cdot k^{-\epsilon}<y<1$.
  By Taylor's theorem there exists  $\zeta\in (\sqrt k\cdot y,\sqrt{k+1}\cdot y)$ such that
  % \begin{align*}
  %   |\sigma_{k+1}(y)-\sigma_k(y)|&=\sigma'(\zeta)\cdot(\sqrt{k+1}-\sqrt k)\cdot y\\
  %   &\leq\sigma'(\zeta)\cdot(\sqrt{k+1}-\sqrt k)\\
  %   &\leq \sigma'(\sqrt k\cdot L\cdot k^{-\epsilon})\cdot(\sqrt{k+1}-\sqrt k)&\sigma'_{|\Real_+}\text{ decreasing}\\
  %   &\leq (1-\sigma(\sqrt k\cdot L\cdot k^{-\epsilon}))\cdot(\sqrt{k+1}-\sqrt k)&\text{\cref{eq:sig2}}\\
  %   &\leq \frac 1{\left(\sqrt k\cdot L\cdot k^{-\epsilon}\right)^2}\cdot(\sqrt{k+1}-\sqrt k)&\text{\cref{lem:sig1}}\\
  %   &\leq \frac 1{\left(\sqrt k\cdot L\cdot k^{-\epsilon}\right)^2}\cdot\frac 1{\sqrt k}&\text{\cref{eq:sqrt}}
  % \end{align*}
  % Otherwise, $y\geq 1$.
  \begin{align*}
    |\sigma_{k+1}(y)-\sigma_k(y)|&=\sigma'(\zeta)\cdot(\sqrt{k+1}-\sqrt k)\cdot y\\
    &\leq \sigma'(\sqrt k\cdot y)\cdot(\sqrt{k+1}-\sqrt k)\cdot y&\sigma'_{|\Real_+}\text{ decreasing}\\
    &\leq (1-\sigma(\sqrt k\cdot y))\cdot(\sqrt{k+1}-\sqrt k)\cdot y&\text{\cref{eq:sig2}}\\
    &\leq \frac 1{\left(\sqrt k\cdot y\right)^2}\cdot(\sqrt{k+1}-\sqrt k)\cdot y&\text{\cref{eq:sigs1}}\\
    &\leq \frac 1{\left(\sqrt k\cdot y\right)^2}\cdot\frac 1{\sqrt k}\cdot y&\text{\cref{eq:sqrt}}\\
    &\leq\frac 1{k\cdot\sqrt k\cdot y} \\
    &\leq\frac 1{k\cdot\sqrt k\cdot L\cdot k^{-\epsilon}}&L\cdot k^{-\epsilon}<y
  \end{align*}
\end{proof}



%\lo{This subsection is mainly about differentiating under the integral sign. It's not clear why it is titled ``unbiasedness''.}
%\dw{It shows that the gradient estimator is unbiased.}

\iffalse
\section{Normalizing Flow}
\dw{integrate in body?}

\lo{The diffeomorphic transformations in the normalising flow framework seem natural examples.}

\begin{example}
\emph{Normalizing flow} \citep{RM15} is a powerful framework for building flexible posterior distributions through an iterative procedure.
It is challenging to enhancing the expressivity of normalising flows since we are constrained by the Jacobians of diffeomorphic transformations, which may be expensive to compute.
Fortunately by introducing dependencies between different dimensions of the latent variables judiciously, we can end up with a tractable Jacobian.
Namely, if after a transformation, dimension $i$ of the resulting variable depends only on dimensions $[1 : i]$ of the input variable, then the Jacobian of this transformation is triangular.
Let $\mu \in \Real^d$ and $\sigma \in \Real^d_{\geq 0}$, define (writing $y_i$ for $\phi_\para(\lat)_i$)
\begin{align*}
y_1 &:= \mu_1 + \sigma_1 \, z_1\\
y_i &:= \mu (y_{1:i-1}) + \sigma (y_{1:i-1}) \, z_1, \quad \hbox{for $i > 1$}
\end{align*}
The Jacobian of this transformation is a lower-triangular matrix with $\sigma(z_{1:i-1})$ on the diagonal;
and the determinant is just the product of the terms on the diagonal.
This is an invertible (and differentiable) transformation, called \emph{autoregressive transformation}:
with the inverse of the form
\[
z_i = \frac{y_i - \mu(y_{1:i-1})}{\sigma(y_{1:i-1})}
\]
\emph{Inverse autoregressive flow} \citep{Kingma2016} is a type of normalising flow that scales well to high-dimensional latent spaces.
The proposed flow consists of a chain of invertible transformations, where each transformation is based on an autoregressive neural network.
The transformed variable is defined as an inverse autoregressive mapping of the following form:
\[
y_i := \sigma(z_{1:i-1}) \, z_i + \mu(z_{1:i-1})
\]
The Jacobian is likewise easy to compute.
\end{example}

\lo{A major recent trend is to extend continuous normalising flows to the discrete setting: \citep {Tran2019,Ziegler2019,Lippe2021,Hoogeboom2019}.
How can our work be applied to problem?}
\fi

\section{Integration by Parts}
\begin{lemma}
  Suppose $f,g\from\Real\times\Real\to\Real$ are smooth. Then for every $\theta\in\Real$,
  \begin{align*}
    \int_{-\infty}^\infty f(\theta,z)\cdot \frac{\partial g}{\partial z}(\theta,z)\diff z=\left[f(\theta,z)\cdot g(\theta,z)\right]^\infty_{-\infty}-\int_{-\infty}^\infty\frac{\partial f}{\partial z}(\theta,z)\cdot g(\theta,z)\diff z
  \end{align*}
\end{lemma}
\begin{proof}
  By the product rule, for every $\theta,z\in\Real$,
  \begin{align*}
    \frac\partial{\partial z}\left(f(\theta,z)\cdot g(\theta,z)\right)=\frac{\partial f}{\partial z}(\theta,z)\cdot g(\theta,z)+f(\theta,z)\cdot\frac{\partial g}{\partial z}(\theta,z)
  \end{align*}
  Therefore, for every $\eta>0$,
  \begin{align*}
    \int_{-\eta}^\eta\frac\partial{\partial z}\left(f(\theta,z)\cdot g(\theta,z)\right)\diff z=\int_{-\eta}^\eta\frac{\partial f}{\partial z}(\theta,z)\cdot g(\theta,z)\diff z+\int_{-\eta}^\eta f(\theta,z)\cdot\frac{\partial g}{\partial z}(\theta,z)\diff z
  \end{align*}
  Besides, for every $\eta>0$,
  \begin{align*}
    \int_{-\eta}^\eta\frac\partial{\partial z}\left(f(\theta,z)\cdot g(\theta,z)\right)\diff z=\left[f(\theta,z)\cdot g(\theta,z)\right]_{-\eta}^\eta
  \end{align*}
  Therefore, provided the limits exist,
  \begin{align*}
    \left[f(\theta,z)\cdot g(\theta,z)\right]_{-\infty}^\infty&=\lim_{\eta\to\infty}\int_{-\eta}^\eta\frac\partial{\partial z}\left(f(\theta,z)\cdot g(\theta,z)\right)\diff z\\
    &=\lim_{\eta\to\infty}\left(\int_{-\eta}^\eta\frac{\partial f}{\partial z}(\theta,z)\cdot g(\theta,z)\diff z+\int_{-\eta}^\eta f(\theta,z)\cdot\frac{\partial g}{\partial z}(\theta,z)\diff z\right)\\
    &=\int_{-\infty}^\infty\frac{\partial f}{\partial z}(\theta,z)\cdot g(\theta,z)\diff z+\int_{-\infty}^\infty f(\theta,z)\cdot\frac{\partial g}{\partial z}(\theta,z)\diff z
  \end{align*}
  and the claim follows.
\end{proof}

\lo{The main thing to check is the reasoning involving ``improper integral''. I see no problem with the proof.}

\begin{corollary}
  Suppose $f,g\from\Real\times\Real\to\Real$ are smooth and that for all $\theta\in\Real$, $\lim_{z\to\pm\infty}(f(\theta,z)\cdot g(\theta,z))=0$. Then for every $\theta\in\Real$,
  \begin{align*}
    \int_{-\infty}^\infty f(\theta,z)\cdot \frac{\partial g}{\partial z}(\theta,z)\diff z=-\int_{-\infty}^\infty\frac{\partial f}{\partial z}(\theta,z)\cdot g(\theta,z)\diff z
  \end{align*}
\end{corollary}

\begin{lemma}
  \label{lem:intp}
  Let $M>0$ and $f,g:\Real\to\Real$ be smooth such that $0\leq f,f'\leq M$, $\lim_{x\to\pm\infty} g(x)=0$ and there is a finite set of disjoint possibly unbounded open intervals $(a_1,b_1),\ldots,(a_m,b_m)$ of $\Real$ such that $g(x)<0$ for $x\in(a_i,b_i)$ and $g(x)\geq 0$ for $x\not\in\bigcup_{i=1}^n(a_i,b_i)$.

  Then $\int |f'(x)\cdot g(x)|\diff x\leq\int |f(x)\cdot g'(x)|\diff x$.
\end{lemma}
\begin{proof}
  Abusing notation, set $b_0\defeq a_{n+1}\defeq\infty$. Note that\footnote{(Ab)using $[-\infty,a_1]\defeq(-\infty,b_1]$ and $[b_n,\infty]\defeq[b_n,\infty)$.} $\Real=\bigcup_{i=1}^n(a_i,b_i)\cup\bigcup_{i=0}^n[b_i,a_{i+1}]$.
  Besides, by continuity and assumption, $f(x)\cdot g(x)=0$ for $x=a_i$ or $x=b_i$ (taking limits for $\pm\infty$).
  Therefore, by partial integration,
  \begin{align*}
    \int_\Real |f'(x)\cdot g(x)|\diff x&=-\sum_{i=1}^n\int_{a_i}^{b_i}f'(x)\cdot g(x)\diff x+\sum_{i=0}^n\int_{b_i}^{a_{i+1}}f'(x)\cdot g(x)\diff x\\
    &=\sum_{i=1}^n\left(\int_{a_i}^{b_i}f(x)\cdot g'(x)\diff x-\underbrace{[f(x)\cdot g(x)]_{a_i}^{b_i}}_0\right)+\sum_{i=0}^n\left(\underbrace{[f(x)\cdot g(x)]_{b_i}^{a_{i+1}}}_0-\int_{b_i}^{a_{i+1}}f(x)\cdot g'(x)\diff x\right)\\
    &\leq\sum_{i=1}^n\int_{a_i}^{b_i}|f(x)\cdot g'(x)|\diff x+\sum_{i=0}^n\int_{b_i}^{a_{i+1}}|f(x)\cdot g'(x)|\diff x=\int_\Real|f(x)\cdot g'(x)|\diff x
  \end{align*}
\end{proof}

\iffalse
We conclude with the following which is very important for the present work:
\begin{corollary}[Integrability]
  \label{cor:int}
  Let $f:\Real^n\to\Real$ be a Schwartz function and $g:\Real^n\to\Real$ be such that $|g|$ is bounded by a polynomial. Then $f\cdot g$ is integrable, i.e.\ $\int |f(\mathbf x)\cdot g(\mathbf x)|\diff\mathbf x<\infty$
\end{corollary}
\fi


\iffalse
\subsection{Uniform Schwartz Functions}


\subsubsection{A Sufficient Criterion}
When is $q_\theta(\repx)=q(\rep_\para^{-1}(\repx))\cdot|\det\Jac\rep_\para(\repx)|$ uniformly Schwartz?
It is sufficient that $q$ is Schwartz, $\rep_{(-)}$ and its partial derivatives is bounded by a polynomial and $\inf_{(\para,\lat)\in\parasp\times\Real^n}\frac{\partial\rep_{(-)}}{\partial s_j}(\para,\lat)>0$. \dw{multivariate} Note that this is a bit stronger than requiring that each $\rep_\para$ is a diffeomorphism.

\changed[dw]{In fact there seems to be a useful bound \cite{H58}: If $p$ is a polynomial with no roots then there exists $c,d>0$ such that $|p(\repx)|>c(1+\|\repx\|^2)^{-d}$. As a consequence, if $f$ is Schwartz and $p$ is a polynomial without roots then $\frac f p$ is Schwartz.}

In particular, this criterion is satisfied for affine transformations $\rep_\para(\lat)=A_\para\cdot\lat+b_\para$, where the components of $A_\para$ and $b_\para$ are polynomially bounded and \dw{$A_\para\neq 0$}
\fi

\section{Old}

\subsection{Uniform Convergence}
\label{sec:unic}

However, even if we can find a stationary point of the smoothed problem, \emph{a priori} it is not obvious the extent to which this is an approximately stationary point of the original problem \eqref{eq:optp}.

Henceforth, we assume that $\parasp\subseteq\Real^m$ is analytic and not constantly $0$.

Note that $0$ is the discontinuity of the Heaviside function and $\sigma_k(0)=\frac 1 2$. Thus, we need to show that applications of sigmoids to $0$ are ``limited''.

If $\psi\from\Real^n\to\Real$ is a non-zero polynomial then the set of arguments which are approximately roots is ``small\footnote{Recall that the set of roots of polynomials is negligible \citep{C05}.}''. Therefore, using the assumption that $\rep_\para$ is a strong diffeomorphism, $\E_{\lat\sim\msnd}[\sigma_{k}(\psi(\rep_\para(\lat)))]$ converges to \changed[dw]{$\E_{\lat\sim\msnd}[[\psi(\rep_\para(\lat))>0]]$}. In fact, the convergence is uniform for $\para\in\parasp$ (\cref{lem:sigsim}).

From this and the fact that, due to compactness of $\parasp$, expectations $\E_\lat[|p_\para(\lat)|]$ can be uniformly bounded for $\para\in\parasp$ it follows relatively straightforwardly (\cref{prop:unic}) that
\begin{align*}
  \E_{\lat\sim\msnd}[\sema k M(\para,\lat)]\xrightarrow{\mathrm{unif}}\E_{\lat\sim\msnd}[\sem M(\para,\lat)]
\end{align*}
as $k\to\infty$ for $\para\in\parasp$.

Proving uniform convergence of gradients is more challenging. The main difficulty is that $\lim_{k\to\infty}\sigma_k'(0)=\infty$ (cf.~\cref{fig:sigd}). Thus, there exist $\para\in\parasp$ and $\lat\in\Real^n$ for which $\nabla_\para\sema k M(\para,\lat)$ is unbounded: \dw{need sample!}
\begin{align*}
  \nabla_\theta\sema k{\ifc{\phi_\theta(z)} { 0} { 1}}(\theta,z)=\sigma'_k(z+\theta)\to\infty
\end{align*}
whenever $\theta=-z$ for $\phi_\theta(z)=z+\theta$.

Fortunately, this effect again only occurs at ``small'' subsets of the latent space. The key technical trick to taming this behaviour is to cast partial derivatives w.r.t.\ the parameters in terms of gradients w.r.t.\ the latent variables and to use integration by parts, thus eliminating derivatives of $\sigma_k$.

\begin{example}
  \label{ex:unic}
   Consider the (typable) term $M$ defined by
  \begin{align*}
    (\lambda x\ldotp (\ifc x{ 0}{(\ifc{x- 1}{ 1}{ 0})})\;\;\\
    (\phi_\theta(\sample))
  \end{align*}
  where $\phi_\theta(z)\defeq c\cdot z+\theta$ and $0\neq c\in\Real$ is a constant.
  Define
  \begin{align*}
    \Psi_k(\alpha)\defeq\sigma_k(\alpha)\cdot \sigma_k(1-\alpha)
  \end{align*}
  and note that $\sema k M(\theta,z)=\Psi_k(\phi_\theta(z))$.
  % Clearly, by the chain rule,
  % \begin{align*}
  %   \frac{\partial(\Psi_k\circ\phi_{(-)})}{\partial\theta}(\theta,z)=\Psi_k'(\phi_\theta(z))\cdot\frac{\partial\phi_{(-)}}{\partial\theta}(\theta,z)
  % \end{align*}
  % Furthermore,
  % \begin{align}
  %   \label{eq:reca}
  %   \frac{\partial\phi_{(-)}}{\partial\theta}(\theta,z)=1=\frac 1 c\cdot\frac{\partial\phi_{(-)}}{\partial z}(\theta,z)
  % \end{align}
  % Therefore,
  By the chain rule we obtain:
  \begin{align}
    \label{eq:extrick}
    \frac{\partial(\Psi_k\circ\phi_{(-)})}{\partial\theta}(\theta,z)=\frac 1 c\cdot\frac{\partial(\Psi_k\circ\phi_{(-)})}{\partial z}(\theta,z)
  \end{align}
  Note that for this it is essential that the guards (which correspond to the factors in the definition of $\Psi_k$) do not depend on the parameters $\theta$, but that they are composed with the same transformation\footnote{in this particular branch of the computation} $\rep_\para$.

  This enables us to employ integration by parts:
  \begin{align*}
    &\E_z\left[\frac{\partial(\Psi_k\circ\phi_{(-)})}{\partial\theta}(\theta,z)\right]\\
    &=\int\nd(z)\cdot\frac 1 c\cdot\frac{\partial(\Psi_k\circ\phi_{(-)})}{\partial z}(\theta,z)\diff z\\
    &=\frac 1 c\left([\nd(z)\cdot \Psi_k(\phi_\theta(z))]_{-\infty}^\infty+\E_z[z\cdot \Psi_k(\phi_\theta(z))]\right)
  \end{align*}
  since $\frac{\partial\nd}{\partial x}(x)=-x\cdot\nd(x)$.
  Due to $0\leq \Psi_k(\phi_\theta(z))\leq 1$ the first summand is $0$ and the uniform convergence of the second follows as above.
\end{example}

The following example illustrates that it is \emph{not} sufficient to restrict terms $\phi_\para(M_1,\ldots,M_\ell,\sample)$ to polynomial \emph{bijections}:
\begin{example}[Divergence]
  \label{ex:div}
  Suppose $M\equiv\ifc{\phi_\theta(\sample)}{ 0}{ 1}$, where $\phi_\theta(z)\defeq z^3+\theta$.
  Note that $\phi_\theta\from\Real\to\Real$ is not a diffeomorphism because $\phi^{-1}_\theta(\alpha)=\sqrt[3]{\alpha-\theta}$ is not differentiable at $\alpha=\theta$.
  Then
  \begin{align*}
    \E_{z\sim\nd(0,1)}[\sem M(\theta,z)]&=\int_{-\sqrt[3]{-\theta}}^\infty\nd(z\mid 0,1)\diff z\\
    \frac\partial{\partial\theta}\E_{z\sim\nd(0,1)}[\sem M(\theta,z)]&=\frac 1 3\cdot \nd(-\sqrt[3]{-\theta}\mid 0,1)\cdot \theta^{-\frac 2 3}
  \end{align*}
  Therefore $\theta\mapsto\E_{z\sim\nd(0,1)}[\sem M(\para,z)]$ is not differentiable at $0$. Besides, for $\theta=0$,
  \begin{align*}
    \E_{z\sim\nd(0,1)}\left[\frac\partial{\partial\theta}\sema k M(\para,z)\right]=\E_{z\sim\nd(0,1)}\left[\sigma_k'(z^3)\right]\to\infty
  \end{align*}
\end{example}

The significance of \cref{prop:unifg} is that it provides the theoretical basis for obtaining approximately stationary points for the original problem \eqref{eq:optp}: given an error tolerance $\epsilon>0$ there exists an accuracy coefficient $k$ such that $\|\nabla_\para\E_{\lat}[\sema k M(\para,\lat)]-\nabla_\para\E_{\lat}[\sem M(\para,\lat)]\|<\epsilon$ for all $\para\in\parasp$. Thus, a stationary point $\para^*\in\parasp$ of the smoothed problem for accuracy coefficient $k$ (which may be obtained by SGD) is approximately stationary: \dw{$\para^*$!!!} \dw{also}
\begin{align*}
  \|\nabla_\para\E_{\lat\sim\msnd}[\sem M(\para^*,\lat)]\|<\epsilon
\end{align*}

\section{Supplementary Materials for \cref{sec:prob}}

\begin{align*}
  \logden(\skipp)&\defeq 0\\
  \logden(x:=F;P)&\defeq \logden(P[F/x])\\
  \logden(z_j\sim\dist(F_1,\ldots,F_k);P)&\defeq \logpdf_{\dist}(z_j\mid F_1,\ldots, F_k)+ \logden(P)\\
  \logden(\observe F {\dist(F_1,\ldots,F_k)};P)&\defeq \logpdf_{\dist}(F\mid F_1,\ldots, F_k)+ \logden(P)
  % \logden(x:=\ifc{E_1}{E_2}{E_3};P)&\defeq\logden(P[\ifc{E_1}{E_2}{E_3}/x])
\end{align*}

\paragraph{Accuracy coefficients for the \textsc{Smooth} estimator}

For the \textsc{Smooth} estimator, for iteration $k \in \mathbb{N}$ we use
% the smoothing coefficient $\eta_k$ \bk{is this defined?} to be $10 \sqrt{k}$ \bk{discuss this value?}.
% \changed[dw]{the slightly modified $\sigma_k(x)\defeq\sigma(10\sqrt k\cdot x)$}.
the slightly modified $\sigma_k(x)\defeq\sigma(10\sqrt k\cdot x)$. The
coefficient (here $10$) was chosen to work well in the experimental setup given.
Larger values resulted in a lower variance for each estimate but ultimately
performed poorer when doing gradient descent with Adam. Intuitively, this comes
from Adam being momentum-based and the a large smoothing value increases the
bias of the initial few gradient estimates which are done on smoother
approximations of the target function.

The experimental results for this on the \texttt{temperature} model are shown in
Figure~\ref{fig:smoothing}.

\begin{figure}
  \centering
  \begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\columnwidth]{figures/smoothing.eps}
  \end{subfigure}
  \caption{Varying the smoothing coefficient on the \texttt{temperature} model.}
  \label{fig:smoothing}
\end{figure}

